Novel Receiver for Superparamagnetic Iron Oxide Nanoparticles in a Molecular Communication Setting

Superparamagnetic iron oxide nanoparticles (SPIONs) have recently been introduced as information carriers in a testbed for molecular communication (MC) in duct flow. Here, a new receiver for this testbed is presented, based on the concept of a bridge circuit. The capability for a reliable transmission using the testbed and detection of the proposed receiver was evaluated by sending a text message and a 80 bit random sequence at a bit rate of 1/s, which resulted in a bit error rate of 0 %. Furthermore, the sensitivity of the device was assessed by a dilution series, which gave a limit for the detectability of peaks between 0.1 to 0.5 mg/mL. Compared to the commercial susceptometer that was previously used as receiver, the new detector provides an increased sampling rate of 100 samples/s and flexibility in the dimensions of the propagation channel. Furthermore, it allows to implement both single-ended and differential signaling in SPION-bases MC testbeds.

==> addplot__Dilution1.tex <==
\addplot [black, thick] coordinates{
		(0,0.173789523809524)
		(0.01,0.173182619047619)
		(0.02,0.173182619047619)
		(0.03,0.173546761904762)
		(0.04,0.173304)
		(0.05,0.172939857142857)
		(0.06,0.173061238095238)
		(0.07,0.173304)
		(0.08,0.172697095238095)
		(0.09,0.172454333333333)
		(0.1,0.172454333333333)
		(0.11,0.172332952380952)
		(0.12,0.172575714285714)
		(0.13,0.172575714285714)
		(0.14,0.172939857142857)
		(0.15,0.173061238095238)
		(0.16,0.172818476190476)
		(0.17,0.172818476190476)
		(0.18,0.172575714285714)
		(0.19,0.173182619047619)
		(0.2,0.172818476190476)
		(0.21,0.172818476190476)
		(0.22,0.173061238095238)
		(0.23,0.173425380952381)
		(0.24,0.173304)
		(0.25,0.173182619047619)
		(0.26,0.172818476190476)
		(0.27,0.172575714285714)
		(0.28,0.172575714285714)
		(0.29,0.173061238095238)
		(0.3,0.173304)
		(0.31,0.173182619047619)
		(0.32,0.173182619047619)
		(0.33,0.172697095238095)
		(0.34,0.173061238095238)
		(0.35,0.172939857142857)
		(0.36,0.172575714285714)
		(0.37,0.172575714285714)
		(0.38,0.173061238095238)
		(0.39,0.173546761904762)
		(0.4,0.172939857142857)
		(0.41,0.173182619047619)
		(0.42,0.173182619047619)
		(0.43,0.172818476190476)
		(0.44,0.172332952380952)
		(0.45,0.172332952380952)
		(0.46,0.172332952380952)
		(0.47,0.172575714285714)
		(0.48,0.172575714285714)
		(0.49,0.172575714285714)
		(0.5,0.172090190476191)
		(0.51,0.172332952380952)
		(0.52,0.172332952380952)
		(0.53,0.172332952380952)
		(0.54,0.172575714285714)
		(0.55,0.171847428571429)
		(0.56,0.172211571428571)
		(0.57,0.172575714285714)
		(0.58,0.172332952380952)
		(0.59,0.172211571428571)
		(0.6,0.172454333333333)
		(0.61,0.172818476190476)
		(0.62,0.172332952380952)
		(0.63,0.172332952380952)
		(0.64,0.173061238095238)
		(0.65,0.172939857142857)
		(0.66,0.172575714285714)
		(0.67,0.173182619047619)
		(0.68,0.173182619047619)
		(0.69,0.173182619047619)
		(0.7,0.173425380952381)
		(0.71,0.173546761904762)
		(0.72,0.173304)
		(0.73,0.173061238095238)
		(0.74,0.173425380952381)
		(0.75,0.173546761904762)
		(0.76,0.173910904761905)
		(0.77,0.173668142857143)
		(0.78,0.173182619047619)
		(0.79,0.173789523809524)
		(0.8,0.174032285714286)
		(0.81,0.173668142857143)
		(0.82,0.174153666666667)
		(0.83,0.174760571428571)
		(0.84,0.175124714285714)
		(0.85,0.174881952380952)
		(0.86,0.175853)
		(0.87,0.176338523809524)
		(0.88,0.176824047619048)
		(0.89,0.177430952380952)
		(0.9,0.177673714285714)
		(0.91,0.177916476190476)
		(0.92,0.178523380952381)
		(0.93,0.179373047619048)
		(0.94,0.179979952380952)
		(0.95,0.180465476190476)
		(0.96,0.180951)
		(0.97,0.181557904761905)
		(0.98,0.182407571428571)
		(0.99,0.183257238095238)
		(1,0.183621380952381)
		(1.01,0.183985523809524)
		(1.02,0.18471380952381)
		(1.03,0.185077952380952)
		(1.04,0.185442095238095)
		(1.05,0.185684857142857)
		(1.06,0.186655904761905)
		(1.07,0.186655904761905)
		(1.08,0.187626952380952)
		(1.09,0.18738419047619)
		(1.1,0.187505571428571)
		(1.11,0.187991095238095)
		(1.12,0.187991095238095)
		(1.13,0.188962142857143)
		(1.14,0.189083523809524)
		(1.15,0.189447666666667)
		(1.16,0.189933190476191)
		(1.17,0.190297333333333)
		(1.18,0.190661476190476)
		(1.19,0.190904238095238)
		(1.2,0.191389761904762)
		(1.21,0.191511142857143)
		(1.22,0.191996666666667)
		(1.23,0.191875285714286)
		(1.24,0.191875285714286)
		(1.25,0.192118047619048)
		(1.26,0.192118047619048)
		(1.27,0.19236080952381)
		(1.28,0.19248219047619)
		(1.29,0.192724952380952)
		(1.3,0.193210476190476)
		(1.31,0.193574619047619)
		(1.32,0.193938761904762)
		(1.33,0.194545666666667)
		(1.34,0.194181523809524)
		(1.35,0.194302904761905)
		(1.36,0.194545666666667)
		(1.37,0.194302904761905)
		(1.38,0.194667047619048)
		(1.39,0.194667047619048)
		(1.4,0.194060142857143)
		(1.41,0.194181523809524)
		(1.42,0.194302904761905)
		(1.43,0.194302904761905)
		(1.44,0.194302904761905)
		(1.45,0.194424285714286)
		(1.46,0.194302904761905)
		(1.47,0.194181523809524)
		(1.48,0.193938761904762)
		(1.49,0.193938761904762)
		(1.5,0.193453238095238)
		(1.51,0.193574619047619)
		(1.52,0.193089095238095)
		(1.53,0.192724952380952)
		(1.54,0.192360809523809)
		(1.55,0.192239428571429)
		(1.56,0.192239428571429)
		(1.57,0.191753904761905)
		(1.58,0.191632523809524)
		(1.59,0.190782857142857)
		(1.6,0.190418714285714)
		(1.61,0.190540095238095)
		(1.62,0.190297333333333)
		(1.63,0.189690428571429)
		(1.64,0.189083523809524)
		(1.65,0.189204904761905)
		(1.66,0.189083523809524)
		(1.67,0.188840761904762)
		(1.68,0.189326285714286)
		(1.69,0.188598)
		(1.7,0.188355238095238)
		(1.71,0.187748333333333)
		(1.72,0.187505571428571)
		(1.73,0.187626952380952)
		(1.74,0.18738419047619)
		(1.75,0.18738419047619)
		(1.76,0.186777285714286)
		(1.77,0.186413142857143)
		(1.78,0.186413142857143)
		(1.79,0.186291761904762)
		(1.8,0.186291761904762)
		(1.81,0.186170380952381)
		(1.82,0.185563476190476)
		(1.83,0.185199333333333)
		(1.84,0.185320714285714)
		(1.85,0.185199333333333)
		(1.86,0.184956571428571)
		(1.87,0.184228285714286)
		(1.88,0.183742761904762)
		(1.89,0.1835)
		(1.9,0.183621380952381)
		(1.91,0.183742761904762)
		(1.92,0.184106904761905)
		(1.93,0.183742761904762)
		(1.94,0.183257238095238)
		(1.95,0.183135857142857)
		(1.96,0.182771714285714)
		(1.97,0.182893095238095)
		(1.98,0.18228619047619)
		(1.99,0.18216480952381)
		(2,0.181679285714286)
		(2.01,0.181557904761905)
		(2.02,0.181315142857143)
		(2.03,0.181315142857143)
		(2.04,0.181315142857143)
		(2.05,0.180951)
		(2.06,0.180829619047619)
		(2.07,0.180708238095238)
		(2.08,0.181193761904762)
		(2.09,0.181072380952381)
		(2.1,0.180708238095238)
		(2.11,0.180586857142857)
		(2.12,0.180222714285714)
		(2.13,0.179979952380952)
		(2.14,0.179858571428571)
		(2.15,0.180101333333333)
		(2.16,0.17973719047619)
		(2.17,0.17973719047619)
		(2.18,0.17973719047619)
		(2.19,0.179615809523809)
		(2.2,0.179858571428571)
		(2.21,0.179494428571429)
		(2.22,0.179494428571429)
		(2.23,0.179251666666667)
		(2.24,0.179494428571429)
		(2.25,0.179251666666667)
		(2.26,0.179251666666667)
		(2.27,0.179494428571429)
		(2.28,0.179494428571429)
		(2.29,0.179251666666667)
		(2.3,0.179858571428571)
		(2.31,0.179494428571429)
		(2.32,0.179373047619048)
		(2.33,0.179130285714286)
		(2.34,0.178766142857143)
		(2.35,0.178887523809524)
		(2.36,0.178523380952381)
		(2.37,0.178766142857143)
		(2.38,0.178644761904762)
		(2.39,0.178402)
		(2.4,0.178644761904762)
		(2.41,0.178523380952381)
		(2.42,0.178766142857143)
		(2.43,0.178402)
		(2.44,0.179008904761905)
		(2.45,0.178766142857143)
		(2.46,0.178402)
		(2.47,0.178280619047619)
		(2.48,0.178280619047619)
		(2.49,0.178159238095238)
		(2.5,0.177916476190476)
		(2.51,0.177795095238095)
		(2.52,0.177795095238095)
		(2.53,0.177673714285714)
		(2.54,0.177552333333333)
		(2.55,0.177795095238095)
		(2.56,0.177309571428571)
		(2.57,0.177430952380952)
		(2.58,0.177430952380952)
		(2.59,0.177066809523809)
		(2.6,0.177552333333333)
		(2.61,0.177552333333333)
		(2.62,0.17718819047619)
		(2.63,0.177309571428571)
		(2.64,0.17718819047619)
		(2.65,0.17706680952381)
		(2.66,0.176824047619048)
		(2.67,0.177430952380952)
		(2.68,0.177309571428571)
		(2.69,0.176702666666667)
		(2.7,0.176945428571429)
		(2.71,0.177066809523809)
		(2.72,0.176459904761905)
		(2.73,0.176945428571429)
		(2.74,0.176702666666667)
		(2.75,0.17718819047619)
		(2.76,0.176945428571429)
		(2.77,0.177430952380952)
		(2.78,0.177309571428571)
		(2.79,0.177430952380952)
		(2.8,0.178280619047619)
		(2.81,0.178037857142857)
		(2.82,0.178159238095238)
		(2.83,0.178887523809524)
		(2.84,0.179494428571429)
		(2.85,0.180222714285714)
		(2.86,0.180222714285714)
		(2.87,0.181193761904762)
		(2.88,0.181315142857143)
		(2.89,0.182043428571429)
		(2.9,0.182650333333333)
		(2.91,0.182771714285714)
		(2.92,0.183621380952381)
		(2.93,0.18483519047619)
		(2.94,0.185442095238095)
		(2.95,0.186534523809524)
		(2.96,0.187020047619048)
		(2.97,0.187991095238095)
		(2.98,0.188598)
		(2.99,0.189447666666667)
		(3,0.190175952380952)
		(3.01,0.190297333333333)
		(3.02,0.190782857142857)
		(3.03,0.191632523809524)
		(3.04,0.191875285714286)
		(3.05,0.191996666666667)
		(3.06,0.192603571428571)
		(3.07,0.193089095238095)
		(3.08,0.192846333333333)
		(3.09,0.193089095238095)
		(3.1,0.193696)
		(3.11,0.193938761904762)
		(3.12,0.194424285714286)
		(3.13,0.194667047619048)
		(3.14,0.194302904761905)
		(3.15,0.194181523809524)
		(3.16,0.193938761904762)
		(3.17,0.194060142857143)
		(3.18,0.193817380952381)
		(3.19,0.193817380952381)
		(3.2,0.193574619047619)
		(3.21,0.193574619047619)
		(3.22,0.193817380952381)
		(3.23,0.194302904761905)
		(3.24,0.194181523809524)
		(3.25,0.194545666666667)
		(3.26,0.19490980952381)
		(3.27,0.194667047619048)
		(3.28,0.195152571428571)
		(3.29,0.195395333333333)
		(3.3,0.195638095238095)
		(3.31,0.195880857142857)
		(3.32,0.195880857142857)
		(3.33,0.195880857142857)
		(3.34,0.195395333333333)
		(3.35,0.195759476190476)
		(3.36,0.195759476190476)
		(3.37,0.195759476190476)
		(3.38,0.195638095238095)
		(3.39,0.196123619047619)
		(3.4,0.195638095238095)
		(3.41,0.196002238095238)
		(3.42,0.195759476190476)
		(3.43,0.195395333333333)
		(3.44,0.195273952380952)
		(3.45,0.195152571428571)
		(3.46,0.19490980952381)
		(3.47,0.194424285714286)
		(3.48,0.194060142857143)
		(3.49,0.193938761904762)
		(3.5,0.193938761904762)
		(3.51,0.193453238095238)
		(3.52,0.19248219047619)
		(3.53,0.192846333333333)
		(3.54,0.192603571428571)
		(3.55,0.192603571428571)
		(3.56,0.192603571428571)
		(3.57,0.19236080952381)
		(3.58,0.19236080952381)
		(3.59,0.19248219047619)
		(3.6,0.191753904761905)
		(3.61,0.192239428571429)
		(3.62,0.191753904761905)
		(3.63,0.191632523809524)
		(3.64,0.191632523809524)
		(3.65,0.191025619047619)
		(3.66,0.190418714285714)
		(3.67,0.18993319047619)
		(3.68,0.189569047619048)
		(3.69,0.189569047619048)
		(3.7,0.188719380952381)
		(3.71,0.188112476190476)
		(3.72,0.187869714285714)
		(3.73,0.188233857142857)
		(3.74,0.187505571428571)
		(3.75,0.186898666666667)
		(3.76,0.186291761904762)
		(3.77,0.185806238095238)
		(3.78,0.185442095238095)
		(3.79,0.185077952380952)
		(3.8,0.184471047619048)
		(3.81,0.18471380952381)
		(3.82,0.184106904761905)
		(3.83,0.183864142857143)
		(3.84,0.183621380952381)
		(3.85,0.183621380952381)
		(3.86,0.183014476190476)
		(3.87,0.183135857142857)
		(3.88,0.182771714285714)
		(3.89,0.182650333333333)
		(3.9,0.182407571428571)
		(3.91,0.182043428571429)
		(3.92,0.182528952380952)
		(3.93,0.182528952380952)
		(3.94,0.18228619047619)
		(3.95,0.181922047619048)
		(3.96,0.182043428571429)
		(3.97,0.181800666666667)
		(3.98,0.181315142857143)
		(3.99,0.181315142857143)
		(4,0.181315142857143)
		(4.01,0.181436523809524)
		(4.02,0.181072380952381)
		(4.03,0.180708238095238)
		(4.04,0.180465476190476)
		(4.05,0.180222714285714)
		(4.06,0.179858571428571)
		(4.07,0.180465476190476)
		(4.08,0.180586857142857)
		(4.09,0.180222714285714)
		(4.1,0.180344095238095)
		(4.11,0.180101333333333)
		(4.12,0.180586857142857)
		(4.13,0.180465476190476)
		(4.14,0.180344095238095)
		(4.15,0.180101333333333)
		(4.16,0.180222714285714)
		(4.17,0.180222714285714)
		(4.18,0.180222714285714)
		(4.19,0.180708238095238)
		(4.2,0.180344095238095)
		(4.21,0.180344095238095)
		(4.22,0.180101333333333)
		(4.23,0.180101333333333)
		(4.24,0.180344095238095)
		(4.25,0.180708238095238)
		(4.26,0.180708238095238)
		(4.27,0.180344095238095)
		(4.28,0.180344095238095)
		(4.29,0.17973719047619)
		(4.3,0.180344095238095)
		(4.31,0.17973719047619)
		(4.32,0.17973719047619)
		(4.33,0.179130285714286)
		(4.34,0.178766142857143)
		(4.35,0.178523380952381)
		(4.36,0.178280619047619)
		(4.37,0.178523380952381)
		(4.38,0.178159238095238)
		(4.39,0.178644761904762)
		(4.4,0.178280619047619)
		(4.41,0.178766142857143)
		(4.42,0.178523380952381)
		(4.43,0.178037857142857)
		(4.44,0.177795095238095)
		(4.45,0.178037857142857)
		(4.46,0.177916476190476)
		(4.47,0.178037857142857)
		(4.48,0.177916476190476)
		(4.49,0.177795095238095)
		(4.5,0.177916476190476)
		(4.51,0.177430952380952)
		(4.52,0.177673714285714)
		(4.53,0.177673714285714)
		(4.54,0.177552333333333)
		(4.55,0.177795095238095)
		(4.56,0.177552333333333)
		(4.57,0.177673714285714)
		(4.58,0.17718819047619)
		(4.59,0.177673714285714)
		(4.6,0.17706680952381)
		(4.61,0.17706680952381)
		(4.62,0.176702666666667)
		(4.63,0.176702666666667)
		(4.64,0.17718819047619)
		(4.65,0.17718819047619)
		(4.66,0.176702666666667)
		(4.67,0.176581285714286)
		(4.68,0.176459904761905)
		(4.69,0.176581285714286)
		(4.7,0.176217142857143)
		(4.71,0.176217142857143)
		(4.72,0.176581285714286)
		(4.73,0.176824047619048)
		(4.74,0.176824047619048)
		(4.75,0.176824047619048)
		(4.76,0.176824047619048)
		(4.77,0.176945428571429)
		(4.78,0.176702666666667)
		(4.79,0.17706680952381)
		(4.8,0.17718819047619)
		(4.81,0.177673714285714)
		(4.82,0.177430952380952)
		(4.83,0.177430952380952)
		(4.84,0.178037857142857)
		(4.85,0.178159238095238)
		(4.86,0.178280619047619)
		(4.87,0.179130285714286)
		(4.88,0.179373047619048)
		(4.89,0.17973719047619)
		(4.9,0.180586857142857)
		(4.91,0.181193761904762)
		(4.92,0.18216480952381)
		(4.93,0.182407571428571)
		(4.94,0.182650333333333)
		(4.95,0.183621380952381)
		(4.96,0.184471047619048)
		(4.97,0.185077952380952)
		(4.98,0.186291761904762)
		(4.99,0.187020047619048)
		(5,0.187505571428571)
		(5.01,0.187748333333333)
		(5.02,0.188112476190476)
		(5.03,0.188840761904762)
		(5.04,0.18993319047619)
		(5.05,0.18993319047619)
		(5.06,0.190418714285714)
		(5.07,0.191147)
		(5.08,0.190782857142857)
		(5.09,0.191389761904762)
		(5.1,0.191753904761905)
		(5.11,0.191875285714286)
		(5.12,0.192360809523809)
		(5.13,0.19248219047619)
		(5.14,0.19236080952381)
		(5.15,0.19236080952381)
		(5.16,0.192239428571429)
		(5.17,0.192846333333333)
		(5.18,0.192603571428571)
		(5.19,0.192967714285714)
		(5.2,0.193331857142857)
		(5.21,0.193696)
		(5.22,0.193696)
		(5.23,0.194060142857143)
		(5.24,0.194424285714286)
		(5.25,0.194302904761905)
		(5.26,0.194545666666667)
		(5.27,0.194302904761905)
		(5.28,0.194667047619048)
		(5.29,0.195395333333333)
		(5.3,0.195395333333333)
		(5.31,0.195152571428571)
		(5.32,0.195395333333333)
		(5.33,0.194788428571429)
		(5.34,0.194545666666667)
		(5.35,0.19490980952381)
		(5.36,0.195273952380952)
		(5.37,0.19503119047619)
		(5.38,0.194667047619048)
		(5.39,0.195152571428571)
		(5.4,0.194545666666667)
		(5.41,0.194667047619048)
		(5.42,0.194424285714286)
		(5.43,0.194788428571429)
		(5.44,0.194667047619048)
		(5.45,0.194667047619048)
		(5.46,0.194545666666667)
		(5.47,0.19490980952381)
		(5.48,0.195395333333333)
		(5.49,0.19503119047619)
		(5.5,0.194667047619048)
		(5.51,0.194545666666667)
		(5.52,0.194909809523809)
		(5.53,0.194788428571429)
		(5.54,0.194667047619048)
		(5.55,0.194424285714286)
		(5.56,0.194545666666667)
		(5.57,0.193817380952381)
		(5.58,0.193817380952381)
		(5.59,0.193453238095238)
		(5.6,0.192603571428571)
		(5.61,0.192724952380952)
		(5.62,0.19248219047619)
		(5.63,0.19248219047619)
		(5.64,0.191753904761905)
		(5.65,0.191753904761905)
		(5.66,0.191389761904762)
		(5.67,0.190782857142857)
		(5.68,0.190175952380952)
		(5.69,0.189569047619048)
		(5.7,0.189326285714286)
		(5.71,0.188719380952381)
		(5.72,0.188476619047619)
		(5.73,0.187748333333333)
		(5.74,0.187020047619048)
		(5.75,0.187141428571429)
		(5.76,0.186534523809524)
		(5.77,0.186291761904762)
		(5.78,0.186049)
		(5.79,0.186170380952381)
		(5.8,0.185806238095238)
		(5.81,0.186049)
		(5.82,0.185563476190476)
		(5.83,0.185442095238095)
		(5.84,0.184592428571429)
		(5.85,0.18471380952381)
		(5.86,0.183864142857143)
		(5.87,0.183621380952381)
		(5.88,0.183621380952381)
		(5.89,0.183135857142857)
		(5.9,0.183257238095238)
		(5.91,0.182650333333333)
		(5.92,0.182650333333333)
		(5.93,0.182407571428571)
		(5.94,0.182407571428571)
		(5.95,0.182650333333333)
		(5.96,0.182043428571429)
		(5.97,0.182650333333333)
		(5.98,0.181800666666667)
		(5.99,0.18216480952381)
		(6,0.181922047619048)
		(6.01,0.182043428571429)
		(6.02,0.181679285714286)
		(6.03,0.181193761904762)
		(6.04,0.180829619047619)
		(6.05,0.181072380952381)
		(6.06,0.180708238095238)
		(6.07,0.181193761904762)
		(6.08,0.180708238095238)
		(6.09,0.180586857142857)
		(6.1,0.180344095238095)
		(6.11,0.180222714285714)
		(6.12,0.180101333333333)
		(6.13,0.180344095238095)
		(6.14,0.180344095238095)
		(6.15,0.180344095238095)
		(6.16,0.179979952380952)
		(6.17,0.180222714285714)
		(6.18,0.179494428571429)
		(6.19,0.180101333333333)
		(6.2,0.17961580952381)
		(6.21,0.179251666666667)
		(6.22,0.179494428571429)
		(6.23,0.179373047619048)
		(6.24,0.17961580952381)
		(6.25,0.179494428571429)
		(6.26,0.17973719047619)
		(6.27,0.179494428571429)
		(6.28,0.178766142857143)
		(6.29,0.179373047619048)
		(6.3,0.179251666666667)
		(6.31,0.179494428571429)
		(6.32,0.179494428571429)
		(6.33,0.17973719047619)
		(6.34,0.17973719047619)
		(6.35,0.179615809523809)
		(6.36,0.179494428571429)
		(6.37,0.17973719047619)
		(6.38,0.17973719047619)
		(6.39,0.17973719047619)
		(6.4,0.179008904761905)
		(6.41,0.179494428571429)
		(6.42,0.17973719047619)
		(6.43,0.179251666666667)
		(6.44,0.179251666666667)
		(6.45,0.179373047619048)
		(6.46,0.179373047619048)
		(6.47,0.178887523809524)
		(6.48,0.179008904761905)
		(6.49,0.179251666666667)
		(6.5,0.179130285714286)
		(6.51,0.179494428571429)
		(6.52,0.179373047619048)
		(6.53,0.178644761904762)
		(6.54,0.178280619047619)
		(6.55,0.177552333333333)
		(6.56,0.177430952380952)
		(6.57,0.177673714285714)
		(6.58,0.177309571428571)
		(6.59,0.177552333333333)
		(6.6,0.177795095238095)
		(6.61,0.178402)
		(6.62,0.177795095238095)
		(6.63,0.177430952380952)
		(6.64,0.177795095238095)
		(6.65,0.177795095238095)
		(6.66,0.177552333333333)
		(6.67,0.17718819047619)
		(6.68,0.17718819047619)
		(6.69,0.177673714285714)
		(6.7,0.177673714285714)
		(6.71,0.17718819047619)
		(6.72,0.17706680952381)
		(6.73,0.176824047619048)
		(6.74,0.17706680952381)
		(6.75,0.177309571428571)
		(6.76,0.177552333333333)
		(6.77,0.177916476190476)
		(6.78,0.177309571428571)
		(6.79,0.177552333333333)
		(6.8,0.17718819047619)
		(6.81,0.17718819047619)
		(6.82,0.176824047619048)
		(6.83,0.177309571428571)
		(6.84,0.177309571428571)
		(6.85,0.177066809523809)
		(6.86,0.176824047619048)
		(6.87,0.176824047619048)
		(6.88,0.176581285714286)
		(6.89,0.176217142857143)
		(6.9,0.175731619047619)
		(6.91,0.175367476190476)
		(6.92,0.175367476190476)
		(6.93,0.175124714285714)
		(6.94,0.175610238095238)
		(6.95,0.175610238095238)
		(6.96,0.175246095238095)
		(6.97,0.175488857142857)
		(6.98,0.175367476190476)
		(6.99,0.175610238095238)
		(7,0.175610238095238)
		(7.01,0.175610238095238)
		(7.02,0.175124714285714)
		(7.03,0.175367476190476)
		(7.04,0.175003333333333)
		(7.05,0.175003333333333)
		(7.06,0.174881952380952)
		(7.07,0.175367476190476)
		(7.08,0.175003333333333)
		(7.09,0.175124714285714)
		(7.1,0.175488857142857)
		(7.11,0.175488857142857)
		(7.12,0.175610238095238)
		(7.13,0.176095761904762)
		(7.14,0.176338523809524)
		(7.15,0.175853)
		(7.16,0.175488857142857)
		(7.17,0.176217142857143)
		(7.18,0.175974380952381)
		(7.19,0.175731619047619)
		(7.2,0.175731619047619)
		(7.21,0.175488857142857)
		(7.22,0.175731619047619)
		(7.23,0.175853)
		(7.24,0.175731619047619)
		(7.25,0.176095761904762)
		(7.26,0.176338523809524)
		(7.27,0.176581285714286)
		(7.28,0.175853)
		(7.29,0.175974380952381)
		(7.3,0.176217142857143)
		(7.31,0.175974380952381)
		(7.32,0.175731619047619)
		(7.33,0.175853)
		(7.34,0.175731619047619)
		(7.35,0.175488857142857)
		(7.36,0.175610238095238)
		(7.37,0.176217142857143)
		(7.38,0.175853)
		(7.39,0.175488857142857)
		(7.4,0.175731619047619)
		(7.41,0.175731619047619)
		(7.42,0.175488857142857)
		(7.43,0.175003333333333)
		(7.44,0.175124714285714)
		(7.45,0.174881952380952)
		(7.46,0.17451780952381)
		(7.47,0.17451780952381)
		(7.48,0.174153666666667)
		(7.49,0.17451780952381)
		(7.5,0.17463919047619)
		(7.51,0.17451780952381)
		(7.52,0.174881952380952)
		(7.53,0.17463919047619)
		(7.54,0.17463919047619)
		(7.55,0.17463919047619)
		(7.56,0.174153666666667)
		(7.57,0.174275047619048)
		(7.58,0.173910904761905)
		(7.59,0.173789523809524)
		(7.6,0.174153666666667)
		(7.61,0.173910904761905)
		(7.62,0.173425380952381)
		(7.63,0.173546761904762)
		(7.64,0.173668142857143)
		(7.65,0.173425380952381)
		(7.66,0.173668142857143)
		(7.67,0.173425380952381)
		(7.68,0.173061238095238)
		(7.69,0.173425380952381)
		(7.7,0.172939857142857)
		(7.71,0.173061238095238)
		(7.72,0.173304)
		(7.73,0.173182619047619)
		(7.74,0.173304)
		(7.75,0.173304)
		(7.76,0.173304)
		(7.77,0.173789523809524)
		(7.78,0.173425380952381)
		(7.79,0.173546761904762)
		(7.8,0.173546761904762)
		(7.81,0.173425380952381)
		(7.82,0.173546761904762)
		(7.83,0.173668142857143)
		(7.84,0.173546761904762)
		(7.85,0.173546761904762)
		(7.86,0.174032285714286)
		(7.87,0.173425380952381)
		(7.88,0.173910904761905)
		(7.89,0.174032285714286)
		(7.9,0.173304)
		(7.91,0.173668142857143)
		(7.92,0.173789523809524)
		(7.93,0.173182619047619)
		(7.94,0.172939857142857)
		(7.95,0.173425380952381)
		(7.96,0.173789523809524)
		(7.97,0.173425380952381)
		(7.98,0.173304)
		(7.99,0.173910904761905)
		(8,0.173425380952381)
		(8.01,0.173425380952381)
		(8.02,0.173425380952381)
		(8.03,0.173668142857143)
		(8.04,0.173910904761905)
		(8.05,0.17451780952381)
		(8.06,0.174517809523809)
		(8.07,0.174032285714286)
		(8.08,0.174760571428571)
		(8.09,0.174396428571429)
		(8.1,0.17451780952381)
		(8.11,0.174881952380952)
		(8.12,0.174760571428571)
		(8.13,0.174275047619048)
		(8.14,0.17463919047619)
		(8.15,0.174760571428571)
		(8.16,0.174396428571429)
		(8.17,0.174396428571429)
		(8.18,0.17463919047619)
		(8.19,0.174396428571429)
		(8.2,0.173668142857143)
		(8.21,0.174032285714286)
		(8.22,0.174032285714286)
		(8.23,0.173910904761905)
		(8.24,0.173425380952381)
		(8.25,0.173546761904762)
		(8.26,0.172818476190476)
		(8.27,0.172818476190476)
		(8.28,0.172697095238095)
		(8.29,0.172454333333333)
		(8.3,0.172575714285714)
		(8.31,0.172332952380952)
		(8.32,0.172090190476191)
		(8.33,0.172332952380952)
		(8.34,0.172939857142857)
		(8.35,0.172575714285714)
		(8.36,0.172575714285714)
		(8.37,0.172454333333333)
		(8.38,0.172332952380952)
		(8.39,0.172454333333333)
		(8.4,0.172454333333333)
		(8.41,0.173061238095238)
		(8.42,0.172697095238095)
		(8.43,0.172697095238095)
		(8.44,0.172575714285714)
		(8.45,0.172697095238095)
		(8.46,0.172211571428571)
		(8.47,0.172454333333333)
		(8.48,0.172211571428571)
		(8.49,0.172575714285714)
		(8.5,0.172818476190476)
		(8.51,0.172818476190476)
		(8.52,0.172818476190476)
		(8.53,0.173425380952381)
		(8.54,0.173304)
		(8.55,0.173182619047619)
		(8.56,0.173910904761905)
		(8.57,0.173910904761905)
		(8.58,0.174032285714286)
		(8.59,0.173789523809524)
		(8.6,0.173425380952381)
		(8.61,0.173546761904762)
		(8.62,0.173425380952381)
		(8.63,0.173546761904762)
		(8.64,0.173789523809524)
		(8.65,0.174396428571429)
		(8.66,0.173910904761905)
		(8.67,0.17451780952381)
		(8.68,0.174275047619048)
		(8.69,0.174760571428571)
		(8.7,0.174517809523809)
		(8.71,0.17451780952381)
		(8.72,0.17451780952381)
		(8.73,0.174639190476191)
		(8.74,0.174275047619048)
		(8.75,0.174275047619048)
		(8.76,0.174275047619048)
		(8.77,0.173910904761905)
		(8.78,0.173789523809524)
		(8.79,0.174275047619048)
		(8.8,0.174275047619048)
		(8.81,0.174275047619048)
		(8.82,0.174760571428571)
		(8.83,0.17463919047619)
		(8.84,0.175124714285714)
		(8.85,0.174881952380952)
		(8.86,0.174881952380952)
		(8.87,0.175367476190476)
		(8.88,0.175124714285714)
		(8.89,0.175124714285714)
		(8.9,0.175124714285714)
		(8.91,0.175003333333333)
		(8.92,0.17463919047619)
		(8.93,0.17463919047619)
		(8.94,0.174153666666667)
		(8.95,0.174153666666667)
		(8.96,0.174153666666667)
		(8.97,0.173668142857143)
		(8.98,0.173546761904762)
		(8.99,0.173668142857143)
		};

==> addplot__Dilution10.tex <==
\addplot [black, thick] coordinates{
		(0,0.203892)
		(0.01,0.204498904761905)
		(0.02,0.204377523809524)
		(0.03,0.204377523809524)
		(0.04,0.204256142857143)
		(0.05,0.204377523809524)
		(0.06,0.204256142857143)
		(0.07,0.203892)
		(0.08,0.204256142857143)
		(0.09,0.204498904761905)
		(0.1,0.204498904761905)
		(0.11,0.204498904761905)
		(0.12,0.204741666666667)
		(0.13,0.204863047619048)
		(0.14,0.204620285714286)
		(0.15,0.204256142857143)
		(0.16,0.203892)
		(0.17,0.203892)
		(0.18,0.204377523809524)
		(0.19,0.204498904761905)
		(0.2,0.204134761904762)
		(0.21,0.204498904761905)
		(0.22,0.204498904761905)
		(0.23,0.204377523809524)
		(0.24,0.204377523809524)
		(0.25,0.204620285714286)
		(0.26,0.204863047619048)
		(0.27,0.204498904761905)
		(0.28,0.204620285714286)
		(0.29,0.204377523809524)
		(0.3,0.204741666666667)
		(0.31,0.204863047619048)
		(0.32,0.204863047619048)
		(0.33,0.204620285714286)
		(0.34,0.204256142857143)
		(0.35,0.204134761904762)
		(0.36,0.204498904761905)
		(0.37,0.204863047619048)
		(0.38,0.20522719047619)
		(0.39,0.205348571428571)
		(0.4,0.205469952380952)
		(0.41,0.206076857142857)
		(0.42,0.205955476190476)
		(0.43,0.205955476190476)
		(0.44,0.206076857142857)
		(0.45,0.206562380952381)
		(0.46,0.206198238095238)
		(0.47,0.205834095238095)
		(0.48,0.206319619047619)
		(0.49,0.206683761904762)
		(0.5,0.206926523809524)
		(0.51,0.206319619047619)
		(0.52,0.206319619047619)
		(0.53,0.206441)
		(0.54,0.206441)
		(0.55,0.206441)
		(0.56,0.206683761904762)
		(0.57,0.206805142857143)
		(0.58,0.206683761904762)
		(0.59,0.206562380952381)
		(0.6,0.206198238095238)
		(0.61,0.205712714285714)
		(0.62,0.20522719047619)
		(0.63,0.205348571428571)
		(0.64,0.205348571428571)
		(0.65,0.205348571428571)
		(0.66,0.205348571428571)
		(0.67,0.205712714285714)
		(0.68,0.206319619047619)
		(0.69,0.207290666666667)
		(0.7,0.208140333333333)
		(0.71,0.208868619047619)
		(0.72,0.210568)
		(0.73,0.212510142857143)
		(0.74,0.214452285714286)
		(0.75,0.216879952380952)
		(0.76,0.219793142857143)
		(0.77,0.222706333333333)
		(0.78,0.22634780952381)
		(0.79,0.23047480952381)
		(0.8,0.234723190476191)
		(0.81,0.239578523809524)
		(0.82,0.245162142857143)
		(0.83,0.251109904761905)
		(0.84,0.256693523809524)
		(0.85,0.262155761904762)
		(0.86,0.267982142857143)
		(0.87,0.274051285714286)
		(0.88,0.28024180952381)
		(0.89,0.286553714285714)
		(0.9,0.293108380952381)
		(0.91,0.30027)
		(0.92,0.308038523809524)
		(0.93,0.315564238095238)
		(0.94,0.323089952380952)
		(0.95,0.330737047619048)
		(0.96,0.337655857142857)
		(0.97,0.343967761904762)
		(0.98,0.350036904761905)
		(0.99,0.355984666666667)
		(1,0.361082761904762)
		(1.01,0.366423619047619)
		(1.02,0.371400285714286)
		(1.03,0.376255571428571)
		(1.04,0.380625333333333)
		(1.05,0.385116476190476)
		(1.06,0.390093142857143)
		(1.07,0.39519119047619)
		(1.08,0.400653428571429)
		(1.09,0.406115666666667)
		(1.1,0.410971)
		(1.11,0.415583571428571)
		(1.12,0.419103666666667)
		(1.13,0.422259619047619)
		(1.14,0.425051428571429)
		(1.15,0.426993523809524)
		(1.16,0.428450095238095)
		(1.17,0.430634952380952)
		(1.18,0.432577047619048)
		(1.19,0.435368857142857)
		(1.2,0.437310952380952)
		(1.21,0.439374428571429)
		(1.22,0.441316571428571)
		(1.23,0.443015904761905)
		(1.24,0.444472476190476)
		(1.25,0.446050476190476)
		(1.26,0.447507047619048)
		(1.27,0.448842285714286)
		(1.28,0.449934761904762)
		(1.29,0.450177523809524)
		(1.3,0.450177523809524)
		(1.31,0.450298904761905)
		(1.32,0.450177523809524)
		(1.33,0.450298904761905)
		(1.34,0.450420285714286)
		(1.35,0.450541666666667)
		(1.36,0.451148619047619)
		(1.37,0.452119714285714)
		(1.38,0.452969428571429)
		(1.39,0.454304666666667)
		(1.4,0.454547428571429)
		(1.41,0.454426047619048)
		(1.42,0.454911619047619)
		(1.43,0.45479019047619)
		(1.44,0.455033)
		(1.45,0.455033)
		(1.46,0.454547428571429)
		(1.47,0.454183285714286)
		(1.48,0.453333571428571)
		(1.49,0.452483857142857)
		(1.5,0.451755523809524)
		(1.51,0.450663047619048)
		(1.52,0.449570571428571)
		(1.53,0.448113952380952)
		(1.54,0.446414571428571)
		(1.55,0.444836571428571)
		(1.56,0.442894428571429)
		(1.57,0.440588142857143)
		(1.58,0.437796333333333)
		(1.59,0.434883142857143)
		(1.6,0.431969952380952)
		(1.61,0.429299523809524)
		(1.62,0.426750523809524)
		(1.63,0.423594571428571)
		(1.64,0.420560047619048)
		(1.65,0.417161333333333)
		(1.66,0.413884047619048)
		(1.67,0.410970904761905)
		(1.68,0.407936380952381)
		(1.69,0.405023238095238)
		(1.7,0.401503142857143)
		(1.71,0.397497523809524)
		(1.72,0.394584333333333)
		(1.73,0.391064238095238)
		(1.74,0.38718)
		(1.75,0.38438819047619)
		(1.76,0.380868095238095)
		(1.77,0.377590761904762)
		(1.78,0.374920333333333)
		(1.79,0.372128523809524)
		(1.8,0.369336714285714)
		(1.81,0.366909047619048)
		(1.82,0.363874476190476)
		(1.83,0.361082666666667)
		(1.84,0.358776380952381)
		(1.85,0.356591476190476)
		(1.86,0.354285190476191)
		(1.87,0.352221666666667)
		(1.88,0.349915380952381)
		(1.89,0.347366333333333)
		(1.9,0.344817285714286)
		(1.91,0.342632428571429)
		(1.92,0.340811714285714)
		(1.93,0.338384095238095)
		(1.94,0.336320619047619)
		(1.95,0.334985428571429)
		(1.96,0.332921952380952)
		(1.97,0.331222619047619)
		(1.98,0.329766047619048)
		(1.99,0.327945333333333)
		(2,0.326246)
		(2.01,0.324546666666667)
		(2.02,0.322847333333333)
		(2.03,0.321390761904762)
		(2.04,0.31957)
		(2.05,0.317627857142857)
		(2.06,0.316171285714286)
		(2.07,0.315078857142857)
		(2.08,0.313136714285714)
		(2.09,0.311437333333333)
		(2.1,0.310466285714286)
		(2.11,0.309131047619048)
		(2.12,0.30779580952381)
		(2.13,0.306339190476191)
		(2.14,0.305003952380952)
		(2.15,0.304032857142857)
		(2.16,0.302697619047619)
		(2.17,0.301726523809524)
		(2.18,0.300148523809524)
		(2.19,0.298691904761905)
		(2.2,0.297356666666667)
		(2.21,0.296749714285714)
		(2.22,0.295778619047619)
		(2.23,0.294079238095238)
		(2.24,0.293350904761905)
		(2.25,0.292744)
		(2.26,0.291772952380952)
		(2.27,0.290316333333333)
		(2.28,0.289102476190476)
		(2.29,0.288738333333333)
		(2.3,0.287888666666667)
		(2.31,0.287038952380952)
		(2.32,0.285825142857143)
		(2.33,0.285218238095238)
		(2.34,0.284854095238095)
		(2.35,0.284611333333333)
		(2.36,0.284004428571429)
		(2.37,0.282912)
		(2.38,0.28157680952381)
		(2.39,0.281212666666667)
		(2.4,0.280848523809524)
		(2.41,0.280241619047619)
		(2.42,0.27914919047619)
		(2.43,0.278420904761905)
		(2.44,0.278056761904762)
		(2.45,0.277449857142857)
		(2.46,0.276964333333333)
		(2.47,0.276357428571429)
		(2.48,0.276114666666667)
		(2.49,0.275386380952381)
		(2.5,0.274172571428571)
		(2.51,0.273444285714286)
		(2.52,0.272473238095238)
		(2.53,0.271987714285714)
		(2.54,0.270773904761905)
		(2.55,0.269924238095238)
		(2.56,0.269074571428571)
		(2.57,0.267739380952381)
		(2.58,0.267011095238095)
		(2.59,0.266768333333333)
		(2.6,0.266040047619048)
		(2.61,0.265069)
		(2.62,0.264097952380952)
		(2.63,0.263612428571429)
		(2.64,0.263005523809524)
		(2.65,0.262762761904762)
		(2.66,0.261670333333333)
		(2.67,0.261063428571429)
		(2.68,0.261306190476191)
		(2.69,0.262155857142857)
		(2.7,0.26373380952381)
		(2.71,0.266282857142857)
		(2.72,0.26943880952381)
		(2.73,0.273201666666667)
		(2.74,0.277328666666667)
		(2.75,0.281577047619048)
		(2.76,0.285704047619048)
		(2.77,0.289345523809524)
		(2.78,0.29420080952381)
		(2.79,0.299056095238095)
		(2.8,0.303304476190476)
		(2.81,0.308159761904762)
		(2.82,0.313864714285714)
		(2.83,0.319569666666667)
		(2.84,0.325396047619048)
		(2.85,0.331586571428571)
		(2.86,0.338019857142857)
		(2.87,0.345060047619048)
		(2.88,0.352464380952381)
		(2.89,0.359504571428571)
		(2.9,0.366180619047619)
		(2.91,0.372128380952381)
		(2.92,0.377226428571429)
		(2.93,0.381353428571429)
		(2.94,0.385480428571429)
		(2.95,0.389000523809524)
		(2.96,0.392884761904762)
		(2.97,0.397011761904762)
		(2.98,0.401745666666667)
		(2.99,0.406115428571429)
		(3,0.410728)
		(3.01,0.415947476190476)
		(3.02,0.42092419047619)
		(3.03,0.425658142857143)
		(3.04,0.430756238095238)
		(3.05,0.435490142857143)
		(3.06,0.439859904761905)
		(3.07,0.443258619047619)
		(3.08,0.446050428571428)
		(3.09,0.448478095238095)
		(3.1,0.450541619047619)
		(3.11,0.452241)
		(3.12,0.454061761904762)
		(3.13,0.455761142857143)
		(3.14,0.45831019047619)
		(3.15,0.459888190476191)
		(3.16,0.462194476190476)
		(3.17,0.464136619047619)
		(3.18,0.466321523809524)
		(3.19,0.468263666666667)
		(3.2,0.469841666666667)
		(3.21,0.471783761904762)
		(3.22,0.473604476190476)
		(3.23,0.474939666666667)
		(3.24,0.475910714285714)
		(3.25,0.476881761904762)
		(3.26,0.478216952380952)
		(3.27,0.479309380952381)
		(3.28,0.480765952380952)
		(3.29,0.483193571428571)
		(3.3,0.485014285714286)
		(3.31,0.486713619047619)
		(3.32,0.48817019047619)
		(3.33,0.489869523809524)
		(3.34,0.491690238095238)
		(3.35,0.493146809523809)
		(3.36,0.494239238095238)
		(3.37,0.494967523809524)
		(3.38,0.49581719047619)
		(3.39,0.496059952380952)
		(3.4,0.496545476190476)
		(3.41,0.496788238095238)
		(3.42,0.496545476190476)
		(3.43,0.49569580952381)
		(3.44,0.495331666666667)
		(3.45,0.494603380952381)
		(3.46,0.493389571428571)
		(3.47,0.491933)
		(3.48,0.490840571428571)
		(3.49,0.489626761904762)
		(3.5,0.487199142857143)
		(3.51,0.484650142857143)
		(3.52,0.482222476190476)
		(3.53,0.479673428571429)
		(3.54,0.476274714285714)
		(3.55,0.473118761904762)
		(3.56,0.469720047619048)
		(3.57,0.466564095238095)
		(3.58,0.463286761904762)
		(3.59,0.459766666666666)
		(3.6,0.45612519047619)
		(3.61,0.452362333333333)
		(3.62,0.448842238095238)
		(3.63,0.445200761904762)
		(3.64,0.441802047619048)
		(3.65,0.437796428571428)
		(3.66,0.43391219047619)
		(3.67,0.429906571428571)
		(3.68,0.42565819047619)
		(3.69,0.421045666666667)
		(3.7,0.417040047619048)
		(3.71,0.413762714285714)
		(3.72,0.410606761904762)
		(3.73,0.407208095238095)
		(3.74,0.404173571428571)
		(3.75,0.401867333333333)
		(3.76,0.399682476190476)
		(3.77,0.397619)
		(3.78,0.395555523809524)
		(3.79,0.393492)
		(3.8,0.391428476190476)
		(3.81,0.389364952380952)
		(3.82,0.387058666666667)
		(3.83,0.384995142857143)
		(3.84,0.382567476190476)
		(3.85,0.379897047619048)
		(3.86,0.377833523809524)
		(3.87,0.376012761904762)
		(3.88,0.374556142857143)
		(3.89,0.373220904761905)
		(3.9,0.371764285714286)
		(3.91,0.370307666666667)
		(3.92,0.368244142857143)
		(3.93,0.366302)
		(3.94,0.365088142857143)
		(3.95,0.363146)
		(3.96,0.361203857142857)
		(3.97,0.359383095238095)
		(3.98,0.357440952380952)
		(3.99,0.35562019047619)
		(4,0.353435333333333)
		(4.01,0.352100142857143)
		(4.02,0.35052219047619)
		(4.03,0.348944238095238)
		(4.04,0.347244904761905)
		(4.05,0.346273857142857)
		(4.06,0.345424190476191)
		(4.07,0.344210380952381)
		(4.08,0.342996571428571)
		(4.09,0.340933095238095)
		(4.1,0.338991)
		(4.11,0.337413047619048)
		(4.12,0.33522819047619)
		(4.13,0.333771619047619)
		(4.14,0.332800571428571)
		(4.15,0.331344)
		(4.16,0.330494333333333)
		(4.17,0.329766047619048)
		(4.18,0.328309476190476)
		(4.19,0.326852904761905)
		(4.2,0.325517714285714)
		(4.21,0.324789428571429)
		(4.22,0.323332857142857)
		(4.23,0.322240428571428)
		(4.24,0.321269380952381)
		(4.25,0.320298333333333)
		(4.26,0.318841761904762)
		(4.27,0.31738519047619)
		(4.28,0.316171380952381)
		(4.29,0.31471480952381)
		(4.3,0.313865095238095)
		(4.31,0.312894)
		(4.32,0.311922904761905)
		(4.33,0.31095180952381)
		(4.34,0.309980714285714)
		(4.35,0.309252428571429)
		(4.36,0.308402761904762)
		(4.37,0.307310285714286)
		(4.38,0.306096428571429)
		(4.39,0.305125333333333)
		(4.4,0.304032857142857)
		(4.41,0.303183142857143)
		(4.42,0.302212047619048)
		(4.43,0.301605095238095)
		(4.44,0.300634)
		(4.45,0.299905666666667)
		(4.46,0.29881319047619)
		(4.47,0.297963476190476)
		(4.48,0.296992380952381)
		(4.49,0.295899904761905)
		(4.5,0.295050190476191)
		(4.51,0.293957761904762)
		(4.52,0.293350857142857)
		(4.53,0.292137047619048)
		(4.54,0.291651523809524)
		(4.55,0.290923238095238)
		(4.56,0.289345238095238)
		(4.57,0.287645857142857)
		(4.58,0.286432047619048)
		(4.59,0.285461)
		(4.6,0.284125809523809)
		(4.61,0.283154761904762)
		(4.62,0.282426476190476)
		(4.63,0.281334047619048)
		(4.64,0.280120238095238)
		(4.65,0.279270571428571)
		(4.66,0.278542285714286)
		(4.67,0.278906428571428)
		(4.68,0.279027809523809)
		(4.69,0.280241666666667)
		(4.7,0.282062428571428)
		(4.71,0.284611476190476)
		(4.72,0.287524666666667)
		(4.73,0.290195095238095)
		(4.74,0.293472428571428)
		(4.75,0.295778714285714)
		(4.76,0.298813285714286)
		(4.77,0.302454761904762)
		(4.78,0.306339)
		(4.79,0.310830142857143)
		(4.8,0.315928238095238)
		(4.81,0.321754619047619)
		(4.82,0.328309285714286)
		(4.83,0.334621190476191)
		(4.84,0.34154)
		(4.85,0.348944333333333)
		(4.86,0.355741761904762)
		(4.87,0.362175047619048)
		(4.88,0.368001428571429)
		(4.89,0.374313333333333)
		(4.9,0.379411380952381)
		(4.91,0.384145285714286)
		(4.92,0.387908142857143)
		(4.93,0.392520666666667)
		(4.94,0.396647666666667)
		(4.95,0.401502952380952)
		(4.96,0.407207952380952)
		(4.97,0.413034333333333)
		(4.98,0.41837519047619)
		(4.99,0.424444333333333)
		(5,0.430027952380952)
		(5.01,0.434640476190476)
		(5.02,0.438646095238095)
		(5.03,0.441437904761905)
		(5.04,0.444472476190476)
		(5.05,0.447021523809524)
		(5.06,0.448842285714286)
		(5.07,0.451512714285714)
		(5.08,0.454304523809524)
		(5.09,0.457096333333333)
		(5.1,0.459524)
		(5.11,0.46243719047619)
		(5.12,0.465593142857143)
		(5.13,0.469113238095238)
		(5.14,0.472147809523809)
		(5.15,0.475425142857143)
		(5.16,0.478338333333333)
		(5.17,0.481251476190476)
		(5.18,0.483557714285714)
		(5.19,0.486106714285714)
		(5.2,0.487684666666667)
		(5.21,0.489262619047619)
		(5.22,0.491204761904762)
		(5.23,0.493389619047619)
		(5.24,0.495574476190476)
		(5.25,0.49739519047619)
		(5.26,0.499337285714286)
		(5.27,0.501643523809524)
		(5.28,0.503464238095238)
		(5.29,0.505406333333333)
		(5.3,0.506862904761905)
		(5.31,0.508076714285714)
		(5.32,0.509533285714286)
		(5.33,0.510625714285714)
		(5.34,0.511111238095238)
		(5.35,0.511718142857143)
		(5.36,0.512325047619048)
		(5.37,0.512325047619048)
		(5.38,0.511596761904762)
		(5.39,0.511354)
		(5.4,0.510504333333333)
		(5.41,0.510504333333333)
		(5.42,0.509654666666667)
		(5.43,0.508198047619048)
		(5.44,0.507227)
		(5.45,0.506134571428572)
		(5.46,0.504678)
		(5.47,0.503100047619048)
		(5.48,0.501279333333334)
		(5.49,0.499337238095238)
		(5.5,0.496909619047619)
		(5.51,0.494724761904762)
		(5.52,0.492539904761905)
		(5.53,0.489990904761905)
		(5.54,0.486956333333333)
		(5.55,0.484285904761905)
		(5.56,0.481251333333333)
		(5.57,0.477974)
		(5.58,0.474818047619048)
		(5.59,0.471783476190476)
		(5.6,0.468384761904762)
		(5.61,0.46535019047619)
		(5.62,0.461951476190476)
		(5.63,0.458916904761905)
		(5.64,0.455882333333333)
		(5.65,0.452240857142857)
		(5.66,0.448963523809524)
		(5.67,0.445807571428571)
		(5.68,0.443137142857143)
		(5.69,0.440223952380952)
		(5.7,0.437553523809524)
		(5.71,0.435004476190476)
		(5.72,0.432819571428571)
		(5.73,0.430513285714286)
		(5.74,0.427842857142857)
		(5.75,0.425172476190476)
		(5.76,0.422623476190476)
		(5.77,0.419831714285714)
		(5.78,0.41679719047619)
		(5.79,0.414369571428571)
		(5.8,0.411577809523809)
		(5.81,0.408664666666667)
		(5.82,0.405751476190476)
		(5.83,0.402716904761905)
		(5.84,0.399925142857143)
		(5.85,0.397376095238095)
		(5.86,0.395312619047619)
		(5.87,0.392884952380952)
		(5.88,0.390700047619048)
		(5.89,0.388151)
		(5.9,0.38535919047619)
		(5.91,0.382567380952381)
		(5.92,0.37965419047619)
		(5.93,0.376498238095238)
		(5.94,0.373706428571428)
		(5.95,0.371278761904762)
		(5.96,0.369093857142857)
		(5.97,0.366787571428571)
		(5.98,0.364602666666667)
		(5.99,0.362781904761905)
		(6,0.360354238095238)
		(6.01,0.358897619047619)
		(6.02,0.356955476190476)
		(6.03,0.355377523809524)
		(6.04,0.35367819047619)
		(6.05,0.351736047619048)
		(6.06,0.349915333333333)
		(6.07,0.347609047619048)
		(6.08,0.345666952380952)
		(6.09,0.343360714285714)
		(6.1,0.34154)
		(6.11,0.340204809523809)
		(6.12,0.338869619047619)
		(6.13,0.337898571428571)
		(6.14,0.336442)
		(6.15,0.33522819047619)
		(6.16,0.334014380952381)
		(6.17,0.333043333333333)
		(6.18,0.331950904761905)
		(6.19,0.330372952380952)
		(6.2,0.329159142857143)
		(6.21,0.327823952380952)
		(6.22,0.325881857142857)
		(6.23,0.324546666666667)
		(6.24,0.323090095238095)
		(6.25,0.321997666666667)
		(6.26,0.320419714285714)
		(6.27,0.319084523809524)
		(6.28,0.318234857142857)
		(6.29,0.317506571428571)
		(6.3,0.316899666666667)
		(6.31,0.315928619047619)
		(6.32,0.31483619047619)
		(6.33,0.313743761904762)
		(6.34,0.312287142857143)
		(6.35,0.311194666666667)
		(6.36,0.310102190476191)
		(6.37,0.308888333333333)
		(6.38,0.307795904761905)
		(6.39,0.306946238095238)
		(6.4,0.306460666666667)
		(6.41,0.305732333333333)
		(6.42,0.305004)
		(6.43,0.304882619047619)
		(6.44,0.304397047619048)
		(6.45,0.303911476190476)
		(6.46,0.303061761904762)
		(6.47,0.302818952380952)
		(6.48,0.302090619047619)
		(6.49,0.301240904761905)
		(6.5,0.300148428571429)
		(6.51,0.299177333333333)
		(6.52,0.297963476190476)
		(6.53,0.297235142857143)
		(6.54,0.296385428571429)
		(6.55,0.295535761904762)
		(6.56,0.295171619047619)
		(6.57,0.294807476190476)
		(6.58,0.293836428571429)
		(6.59,0.292865333333333)
		(6.6,0.291894238095238)
		(6.61,0.29080180952381)
		(6.62,0.289952142857143)
		(6.63,0.289588)
		(6.64,0.288616904761905)
		(6.65,0.287645857142857)
		(6.66,0.286553428571429)
		(6.67,0.285582380952381)
		(6.68,0.284368571428571)
		(6.69,0.283640285714286)
		(6.7,0.282790619047619)
		(6.71,0.282305095238095)
		(6.72,0.281819571428571)
		(6.73,0.281212666666667)
		(6.74,0.280484380952381)
		(6.75,0.279998857142857)
		(6.76,0.279756095238095)
		(6.77,0.279513333333333)
		(6.78,0.278785047619048)
		(6.79,0.278542285714286)
		(6.8,0.278299523809524)
		(6.81,0.277449857142857)
		(6.82,0.277328476190476)
		(6.83,0.276842952380952)
		(6.84,0.275750523809524)
		(6.85,0.275143619047619)
		(6.86,0.274536714285714)
		(6.87,0.274172571428571)
		(6.88,0.273687047619048)
		(6.89,0.273201523809524)
		(6.9,0.272958761904762)
		(6.91,0.272351857142857)
		(6.92,0.271380809523809)
		(6.93,0.270773904761905)
		(6.94,0.270895285714286)
		(6.95,0.270288380952381)
		(6.96,0.269802857142857)
		(6.97,0.269074571428571)
		(6.98,0.268224904761905)
		(6.99,0.267618)
		(7,0.267375238095238)
		(7.01,0.267011095238095)
		(7.02,0.266646952380952)
		(7.03,0.266040047619048)
		(7.04,0.265554523809524)
		(7.05,0.265433142857143)
		(7.06,0.264826238095238)
		(7.07,0.264219333333333)
		(7.08,0.26385519047619)
		(7.09,0.263612428571429)
		(7.1,0.26373380952381)
		(7.11,0.263369666666667)
		(7.12,0.263126904761905)
		(7.13,0.263005523809524)
		(7.14,0.262641380952381)
		(7.15,0.261791714285714)
		(7.16,0.26118480952381)
		(7.17,0.260577904761905)
		(7.18,0.260213761904762)
		(7.19,0.260092380952381)
		(7.2,0.259971)
		(7.21,0.259606857142857)
		(7.22,0.258878571428572)
		(7.23,0.25863580952381)
		(7.24,0.258271666666667)
		(7.25,0.257907523809524)
		(7.26,0.257907523809524)
		(7.27,0.257786142857143)
		(7.28,0.257543380952381)
		(7.29,0.257422)
		(7.3,0.257057857142857)
		(7.31,0.256693714285714)
		(7.32,0.25608680952381)
		(7.33,0.255844047619048)
		(7.34,0.255358523809524)
		(7.35,0.254873)
		(7.36,0.254994380952381)
		(7.37,0.255358523809524)
		(7.38,0.255358523809524)
		(7.39,0.255115761904762)
		(7.4,0.254873)
		(7.41,0.254630238095238)
		(7.42,0.254144714285714)
		(7.43,0.253901952380952)
		(7.44,0.253537809523809)
		(7.45,0.253295047619048)
		(7.46,0.253052285714286)
		(7.47,0.252809523809524)
		(7.48,0.252809523809524)
		(7.49,0.253052285714286)
		(7.5,0.252809523809524)
		(7.51,0.252809523809524)
		(7.52,0.252324)
		(7.53,0.251838476190476)
		(7.54,0.251231571428571)
		(7.55,0.251352952380952)
		(7.56,0.251717095238095)
		(7.57,0.251474333333333)
		(7.58,0.251352952380952)
		(7.59,0.25098880952381)
		(7.6,0.251231571428571)
		(7.61,0.250746047619048)
		(7.62,0.250260523809524)
		(7.63,0.249896380952381)
		(7.64,0.249532238095238)
		(7.65,0.249410857142857)
		(7.66,0.248925333333333)
		(7.67,0.248803952380952)
		(7.68,0.24843980952381)
		(7.69,0.248318428571429)
		(7.7,0.248075666666667)
		(7.71,0.247590142857143)
		(7.72,0.246983238095238)
		(7.73,0.246619095238095)
		(7.74,0.246497714285714)
		(7.75,0.246254952380952)
		(7.76,0.245648047619048)
		(7.77,0.245041142857143)
		(7.78,0.244434238095238)
		(7.79,0.243584571428571)
		(7.8,0.243220428571429)
		(7.81,0.242492142857143)
		(7.82,0.242370761904762)
		(7.83,0.241885238095238)
		(7.84,0.241885238095238)
		(7.85,0.241885238095238)
		(7.86,0.241885238095238)
		(7.87,0.242006619047619)
		(7.88,0.241763857142857)
		(7.89,0.241642476190476)
		(7.9,0.241399714285714)
		(7.91,0.241399714285714)
		(7.92,0.241278333333333)
		(7.93,0.241642476190476)
		(7.94,0.241885238095238)
		(7.95,0.242249380952381)
		(7.96,0.242734904761905)
		(7.97,0.242977666666667)
		(7.98,0.242856285714286)
		(7.99,0.243220428571429)
		(8,0.24334180952381)
		(8.01,0.243705952380952)
		(8.02,0.243827333333333)
		(8.03,0.243584571428571)
		(8.04,0.243705952380952)
		(8.05,0.243584571428571)
		(8.06,0.243220428571429)
		(8.07,0.243099047619048)
		(8.08,0.242856285714286)
		(8.09,0.242492142857143)
		(8.1,0.241763857142857)
		(8.11,0.241156952380952)
		(8.12,0.240307285714286)
		(8.13,0.239943142857143)
		(8.14,0.239336238095238)
		(8.15,0.238972095238095)
		(8.16,0.23836519047619)
		(8.17,0.237879666666667)
		(8.18,0.238001047619048)
		(8.19,0.237879666666667)
		(8.2,0.237394142857143)
		(8.21,0.236908571428571)
		(8.22,0.23678719047619)
		(8.23,0.23666580952381)
		(8.24,0.236544428571429)
		(8.25,0.236180285714286)
		(8.26,0.236058904761905)
		(8.27,0.236544428571429)
		(8.28,0.236423047619048)
		(8.29,0.236301666666667)
		(8.3,0.236301666666667)
		(8.31,0.236544428571429)
		(8.32,0.23666580952381)
		(8.33,0.236544380952381)
		(8.34,0.236423)
		(8.35,0.236423)
		(8.36,0.236665761904762)
		(8.37,0.237029904761905)
		(8.38,0.237272666666667)
		(8.39,0.236908523809524)
		(8.4,0.237029904761905)
		(8.41,0.237272666666667)
		(8.42,0.237879619047619)
		(8.43,0.237758238095238)
		(8.44,0.237636857142857)
		(8.45,0.237272666666667)
		(8.46,0.237029857142857)
		(8.47,0.236908476190476)
		(8.48,0.236422952380952)
		(8.49,0.236422952380952)
		(8.5,0.236665714285714)
		(8.51,0.236787095238095)
		(8.52,0.236908476190476)
		(8.53,0.236787095238095)
		(8.54,0.236665714285714)
		(8.55,0.236422904761905)
		(8.56,0.236058714285714)
		(8.57,0.235330380952381)
		(8.58,0.235087619047619)
		(8.59,0.234723476190476)
		(8.6,0.234723476190476)
		(8.61,0.234723476190476)
		(8.62,0.233995142857143)
		(8.63,0.233509619047619)
		(8.64,0.233145476190476)
		(8.65,0.233388238095238)
		(8.66,0.233266857142857)
		(8.67,0.233266857142857)
		(8.68,0.233145476190476)
		(8.69,0.233024095238095)
		(8.7,0.232538523809524)
		(8.71,0.232174380952381)
		(8.72,0.231931619047619)
		(8.73,0.231567476190476)
		(8.74,0.231324666666667)
		(8.75,0.231810238095238)
		(8.76,0.231688857142857)
		(8.77,0.231688857142857)
		(8.78,0.232174428571429)
		(8.79,0.232053047619048)
		(8.8,0.231688857142857)
		(8.81,0.231688857142857)
		(8.82,0.231567476190476)
		(8.83,0.232053047619048)
		(8.84,0.232053047619048)
		(8.85,0.23229580952381)
		(8.86,0.231810238095238)
		(8.87,0.231810238095238)
		(8.88,0.231688857142857)
		(8.89,0.231567428571429)
		(8.9,0.231203238095238)
		(8.91,0.231081857142857)
		(8.92,0.230839047619048)
		(8.93,0.231081809523809)
		(8.94,0.230960380952381)
		(8.95,0.230717619047619)
		(8.96,0.230474857142857)
		(8.97,0.230717619047619)
		(8.98,0.230596238095238)
		(8.99,0.230232047619048)
		};

==> addplot__Dilution5.tex <==
\addplot [black, thick] coordinates{
		(0,0.18471380952381)
		(0.01,0.18483519047619)
		(0.02,0.184471047619048)
		(0.03,0.183985523809524)
		(0.04,0.184228285714286)
		(0.05,0.184592428571429)
		(0.06,0.184471047619048)
		(0.07,0.184471047619048)
		(0.08,0.18483519047619)
		(0.09,0.185199333333333)
		(0.1,0.185442095238095)
		(0.11,0.185442095238095)
		(0.12,0.185806238095238)
		(0.13,0.186170380952381)
		(0.14,0.186291761904762)
		(0.15,0.186534523809524)
		(0.16,0.186049)
		(0.17,0.185806238095238)
		(0.18,0.185442095238095)
		(0.19,0.185806238095238)
		(0.2,0.185563476190476)
		(0.21,0.185927619047619)
		(0.22,0.186291761904762)
		(0.23,0.186291761904762)
		(0.24,0.186291761904762)
		(0.25,0.185927619047619)
		(0.26,0.185563476190476)
		(0.27,0.185563476190476)
		(0.28,0.185077952380952)
		(0.29,0.184349666666667)
		(0.3,0.183621380952381)
		(0.31,0.183014476190476)
		(0.32,0.183014476190476)
		(0.33,0.183135857142857)
		(0.34,0.183135857142857)
		(0.35,0.183257238095238)
		(0.36,0.182771714285714)
		(0.37,0.183621380952381)
		(0.38,0.183864142857143)
		(0.39,0.183864142857143)
		(0.4,0.1835)
		(0.41,0.183985523809524)
		(0.42,0.184228285714286)
		(0.43,0.184106904761905)
		(0.44,0.184106904761905)
		(0.45,0.184106904761905)
		(0.46,0.184349666666667)
		(0.47,0.18471380952381)
		(0.48,0.184956571428571)
		(0.49,0.184835190476191)
		(0.5,0.185563476190476)
		(0.51,0.185927619047619)
		(0.52,0.186291761904762)
		(0.53,0.186534523809524)
		(0.54,0.186170380952381)
		(0.55,0.186170380952381)
		(0.56,0.185806238095238)
		(0.57,0.186170380952381)
		(0.58,0.185927619047619)
		(0.59,0.185927619047619)
		(0.6,0.186291761904762)
		(0.61,0.185927619047619)
		(0.62,0.186049)
		(0.63,0.185806238095238)
		(0.64,0.185684857142857)
		(0.65,0.186049)
		(0.66,0.186170380952381)
		(0.67,0.185806238095238)
		(0.68,0.185442095238095)
		(0.69,0.185684857142857)
		(0.7,0.186170380952381)
		(0.71,0.186413142857143)
		(0.72,0.187141428571429)
		(0.73,0.188112476190476)
		(0.74,0.189083523809524)
		(0.75,0.190540095238095)
		(0.76,0.191996666666667)
		(0.77,0.194302904761905)
		(0.78,0.196002238095238)
		(0.79,0.19758019047619)
		(0.8,0.199400904761905)
		(0.81,0.201221619047619)
		(0.82,0.203406476190476)
		(0.83,0.205348571428571)
		(0.84,0.207169285714286)
		(0.85,0.209961095238095)
		(0.86,0.212024619047619)
		(0.87,0.215301952380952)
		(0.88,0.218336523809524)
		(0.89,0.222099380952381)
		(0.9,0.225376714285714)
		(0.91,0.228775428571429)
		(0.92,0.232174142857143)
		(0.93,0.235087333333333)
		(0.94,0.237757761904762)
		(0.95,0.240670952380952)
		(0.96,0.242734476190476)
		(0.97,0.244555238095238)
		(0.98,0.246011857142857)
		(0.99,0.247468476190476)
		(1,0.249653380952381)
		(1.01,0.251716904761905)
		(1.02,0.253780428571429)
		(1.03,0.256693619047619)
		(1.04,0.258999904761905)
		(1.05,0.262034476190476)
		(1.06,0.264219333333333)
		(1.07,0.266525571428571)
		(1.08,0.268103523809524)
		(1.09,0.270288380952381)
		(1.1,0.271016666666667)
		(1.11,0.271744952380952)
		(1.12,0.272594619047619)
		(1.13,0.273201523809524)
		(1.14,0.27392980952381)
		(1.15,0.274900857142857)
		(1.16,0.275871904761905)
		(1.17,0.277085714285714)
		(1.18,0.278542285714286)
		(1.19,0.279998857142857)
		(1.2,0.282062333333333)
		(1.21,0.283154761904762)
		(1.22,0.284854142857143)
		(1.23,0.286067952380952)
		(1.24,0.286432095238095)
		(1.25,0.287767333333333)
		(1.26,0.288617047619048)
		(1.27,0.288738428571429)
		(1.28,0.289223952380952)
		(1.29,0.289588095238095)
		(1.3,0.289709476190476)
		(1.31,0.290680523809524)
		(1.32,0.291287428571428)
		(1.33,0.291772952380952)
		(1.34,0.292379857142857)
		(1.35,0.292986761904762)
		(1.36,0.292744)
		(1.37,0.292865380952381)
		(1.38,0.292865380952381)
		(1.39,0.292258476190476)
		(1.4,0.292137095238095)
		(1.41,0.291408809523809)
		(1.42,0.290680523809524)
		(1.43,0.28995219047619)
		(1.44,0.288981142857143)
		(1.45,0.288738380952381)
		(1.46,0.287281761904762)
		(1.47,0.285825142857143)
		(1.48,0.285096857142857)
		(1.49,0.283761666666667)
		(1.5,0.282426476190476)
		(1.51,0.281091285714286)
		(1.52,0.27914919047619)
		(1.53,0.277814)
		(1.54,0.276236047619048)
		(1.55,0.274536714285714)
		(1.56,0.273201523809524)
		(1.57,0.272473238095238)
		(1.58,0.270652523809524)
		(1.59,0.268831809523809)
		(1.6,0.267253857142857)
		(1.61,0.265797285714286)
		(1.62,0.264219333333333)
		(1.63,0.262641380952381)
		(1.64,0.260699285714286)
		(1.65,0.259242714285714)
		(1.66,0.256815095238095)
		(1.67,0.255479904761905)
		(1.68,0.254144714285714)
		(1.69,0.252809523809524)
		(1.7,0.251717095238095)
		(1.71,0.250260523809524)
		(1.72,0.248925333333333)
		(1.73,0.247832904761905)
		(1.74,0.246861857142857)
		(1.75,0.245769428571429)
		(1.76,0.24431280952381)
		(1.77,0.242977619047619)
		(1.78,0.241521047619048)
		(1.79,0.24030719047619)
		(1.8,0.239336095238095)
		(1.81,0.238971952380952)
		(1.82,0.237758095238095)
		(1.83,0.236908380952381)
		(1.84,0.236301428571428)
		(1.85,0.235451714285714)
		(1.86,0.234723380952381)
		(1.87,0.23435919047619)
		(1.88,0.233388095238095)
		(1.89,0.232295619047619)
		(1.9,0.231324523809524)
		(1.91,0.23047480952381)
		(1.92,0.229625095238095)
		(1.93,0.229260904761905)
		(1.94,0.228653952380952)
		(1.95,0.227561476190476)
		(1.96,0.227318666666667)
		(1.97,0.227075904761905)
		(1.98,0.226711714285714)
		(1.99,0.226226142857143)
		(2,0.226226142857143)
		(2.01,0.225740619047619)
		(2.02,0.225012285714286)
		(2.03,0.224648142857143)
		(2.04,0.223919857142857)
		(2.05,0.223798476190476)
		(2.06,0.223312952380952)
		(2.07,0.222827428571429)
		(2.08,0.222220523809524)
		(2.09,0.221977761904762)
		(2.1,0.221249476190476)
		(2.11,0.220642571428571)
		(2.12,0.220278428571429)
		(2.13,0.219792904761905)
		(2.14,0.219064619047619)
		(2.15,0.219064619047619)
		(2.16,0.218457714285714)
		(2.17,0.21785080952381)
		(2.18,0.217486666666667)
		(2.19,0.216879761904762)
		(2.2,0.216394238095238)
		(2.21,0.215665952380952)
		(2.22,0.21530180952381)
		(2.23,0.215059047619048)
		(2.24,0.214330761904762)
		(2.25,0.214088)
		(2.26,0.213359714285714)
		(2.27,0.212995571428571)
		(2.28,0.212631428571429)
		(2.29,0.212510047619048)
		(2.3,0.212145904761905)
		(2.31,0.211903142857143)
		(2.32,0.211660380952381)
		(2.33,0.211660380952381)
		(2.34,0.211417619047619)
		(2.35,0.211417619047619)
		(2.36,0.210689333333333)
		(2.37,0.210689333333333)
		(2.38,0.210203809523809)
		(2.39,0.209839666666667)
		(2.4,0.209839666666667)
		(2.41,0.209354142857143)
		(2.42,0.209111380952381)
		(2.43,0.209111380952381)
		(2.44,0.208625857142857)
		(2.45,0.208383095238095)
		(2.46,0.208383095238095)
		(2.47,0.208383095238095)
		(2.48,0.208383095238095)
		(2.49,0.208504476190476)
		(2.5,0.208140333333333)
		(2.51,0.207533428571429)
		(2.52,0.207897571428571)
		(2.53,0.20765480952381)
		(2.54,0.206805142857143)
		(2.55,0.206926523809524)
		(2.56,0.206562380952381)
		(2.57,0.206683761904762)
		(2.58,0.206562380952381)
		(2.59,0.206319619047619)
		(2.6,0.205834095238095)
		(2.61,0.205469952380952)
		(2.62,0.205834095238095)
		(2.63,0.205834095238095)
		(2.64,0.205591333333333)
		(2.65,0.205105809523809)
		(2.66,0.205348571428571)
		(2.67,0.20522719047619)
		(2.68,0.204741666666667)
		(2.69,0.204256142857143)
		(2.7,0.203892)
		(2.71,0.203770619047619)
		(2.72,0.203892)
		(2.73,0.203649238095238)
		(2.74,0.204134761904762)
		(2.75,0.20510580952381)
		(2.76,0.206319666666667)
		(2.77,0.207776285714286)
		(2.78,0.208868761904762)
		(2.79,0.20996119047619)
		(2.8,0.212024714285714)
		(2.81,0.213966857142857)
		(2.82,0.215666238095238)
		(2.83,0.218093904761905)
		(2.84,0.220764333333333)
		(2.85,0.223556142857143)
		(2.86,0.227076238095238)
		(2.87,0.230353571428571)
		(2.88,0.233873666666667)
		(2.89,0.237515142857143)
		(2.9,0.240671095238095)
		(2.91,0.243462904761905)
		(2.92,0.246497476190476)
		(2.93,0.249289285714286)
		(2.94,0.252202476190476)
		(2.95,0.254994285714286)
		(2.96,0.257664714285714)
		(2.97,0.260213714285714)
		(2.98,0.262641333333333)
		(2.99,0.265797238095238)
		(3,0.26883180952381)
		(3.01,0.271259428571429)
		(3.02,0.274415380952381)
		(3.03,0.276964380952381)
		(3.04,0.278299571428571)
		(3.05,0.279998904761905)
		(3.06,0.281334095238095)
		(3.07,0.282426523809524)
		(3.08,0.28315480952381)
		(3.09,0.28327619047619)
		(3.1,0.283518952380952)
		(3.11,0.284611380952381)
		(3.12,0.285946571428571)
		(3.13,0.287767333333333)
		(3.14,0.289952238095238)
		(3.15,0.292015761904762)
		(3.16,0.293715142857143)
		(3.17,0.295414523809524)
		(3.18,0.296385619047619)
		(3.19,0.297235333333333)
		(3.2,0.297720904761905)
		(3.21,0.298570619047619)
		(3.22,0.298570619047619)
		(3.23,0.298327809523809)
		(3.24,0.298692)
		(3.25,0.299056142857143)
		(3.26,0.298570619047619)
		(3.27,0.298692)
		(3.28,0.298570619047619)
		(3.29,0.298813380952381)
		(3.3,0.299663047619048)
		(3.31,0.300634142857143)
		(3.32,0.300755523809524)
		(3.33,0.300755523809524)
		(3.34,0.300512714285714)
		(3.35,0.300148523809524)
		(3.36,0.299905761904762)
		(3.37,0.299541571428571)
		(3.38,0.298934619047619)
		(3.39,0.298691809523809)
		(3.4,0.29881319047619)
		(3.41,0.298327619047619)
		(3.42,0.297963428571428)
		(3.43,0.29820619047619)
		(3.44,0.297963428571429)
		(3.45,0.296870952380952)
		(3.46,0.296385428571429)
		(3.47,0.29650680952381)
		(3.48,0.296142666666667)
		(3.49,0.295778523809524)
		(3.5,0.294928857142857)
		(3.51,0.293836428571429)
		(3.52,0.29250119047619)
		(3.53,0.291651523809524)
		(3.54,0.290559095238095)
		(3.55,0.289466666666667)
		(3.56,0.287645952380952)
		(3.57,0.285582428571429)
		(3.58,0.284125857142857)
		(3.59,0.282669285714286)
		(3.6,0.280363047619048)
		(3.61,0.278056761904762)
		(3.62,0.27647880952381)
		(3.63,0.274415333333333)
		(3.64,0.272109095238095)
		(3.65,0.270531142857143)
		(3.66,0.269317333333333)
		(3.67,0.267739380952381)
		(3.68,0.266040047619048)
		(3.69,0.264704857142857)
		(3.7,0.263248285714286)
		(3.71,0.261670333333333)
		(3.72,0.260213761904762)
		(3.73,0.258514428571429)
		(3.74,0.257300619047619)
		(3.75,0.256086809523809)
		(3.76,0.254508857142857)
		(3.77,0.253780571428571)
		(3.78,0.252445380952381)
		(3.79,0.251352952380952)
		(3.8,0.249653619047619)
		(3.81,0.248925333333333)
		(3.82,0.248197047619048)
		(3.83,0.246861857142857)
		(3.84,0.245890809523809)
		(3.85,0.245041142857143)
		(3.86,0.244191476190476)
		(3.87,0.243099047619048)
		(3.88,0.242128)
		(3.89,0.241278333333333)
		(3.9,0.240185904761905)
		(3.91,0.238972047619048)
		(3.92,0.238243714285714)
		(3.93,0.237515428571429)
		(3.94,0.236908476190476)
		(3.95,0.235937380952381)
		(3.96,0.235330428571429)
		(3.97,0.234480714285714)
		(3.98,0.233509619047619)
		(3.99,0.233266809523809)
		(4,0.232295714285714)
		(4.01,0.231688761904762)
		(4.02,0.231324571428571)
		(4.03,0.230353476190476)
		(4.04,0.229989285714286)
		(4.05,0.229625095238095)
		(4.06,0.229018142857143)
		(4.07,0.228047047619048)
		(4.08,0.227804238095238)
		(4.09,0.227318666666667)
		(4.1,0.226590333333333)
		(4.11,0.226104761904762)
		(4.12,0.226104761904762)
		(4.13,0.225376476190476)
		(4.14,0.224890904761905)
		(4.15,0.224526761904762)
		(4.16,0.223919857142857)
		(4.17,0.22307019047619)
		(4.18,0.22294880952381)
		(4.19,0.222827428571429)
		(4.2,0.222341904761905)
		(4.21,0.221492238095238)
		(4.22,0.221249476190476)
		(4.23,0.220885333333333)
		(4.24,0.220763952380952)
		(4.25,0.220035666666667)
		(4.26,0.219671523809524)
		(4.27,0.219671523809524)
		(4.28,0.219307380952381)
		(4.29,0.218821857142857)
		(4.3,0.218457714285714)
		(4.31,0.218336333333333)
		(4.32,0.218214952380952)
		(4.33,0.217608047619048)
		(4.34,0.217608047619048)
		(4.35,0.217486666666667)
		(4.36,0.216879761904762)
		(4.37,0.216879761904762)
		(4.38,0.217001142857143)
		(4.39,0.216515619047619)
		(4.4,0.215908714285714)
		(4.41,0.215787333333333)
		(4.42,0.215665952380952)
		(4.43,0.215787333333333)
		(4.44,0.215180428571429)
		(4.45,0.214694904761905)
		(4.46,0.214452142857143)
		(4.47,0.213845238095238)
		(4.48,0.213238333333333)
		(4.49,0.212995571428571)
		(4.5,0.212631428571429)
		(4.51,0.212388666666667)
		(4.52,0.211781761904762)
		(4.53,0.211053476190476)
		(4.54,0.210810714285714)
		(4.55,0.210810714285714)
		(4.56,0.209961047619048)
		(4.57,0.209961047619048)
		(4.58,0.209718285714286)
		(4.59,0.209475523809524)
		(4.6,0.209475523809524)
		(4.61,0.20899)
		(4.62,0.208383095238095)
		(4.63,0.208140333333333)
		(4.64,0.20765480952381)
		(4.65,0.207169285714286)
		(4.66,0.206805142857143)
		(4.67,0.206805142857143)
		(4.68,0.206562380952381)
		(4.69,0.206076857142857)
		(4.7,0.205955476190476)
		(4.71,0.205955476190476)
		(4.72,0.205469952380952)
		(4.73,0.205712714285714)
		(4.74,0.205834095238095)
		(4.75,0.205955476190476)
		(4.76,0.206076857142857)
		(4.77,0.207047904761905)
		(4.78,0.208504523809524)
		(4.79,0.209839761904762)
		(4.8,0.211903285714286)
		(4.81,0.21396680952381)
		(4.82,0.216394476190476)
		(4.83,0.219064904761905)
		(4.84,0.221735333333333)
		(4.85,0.223920238095238)
		(4.86,0.226712047619048)
		(4.87,0.229261095238095)
		(4.88,0.231324619047619)
		(4.89,0.233995047619048)
		(4.9,0.237393761904762)
		(4.91,0.240306952380952)
		(4.92,0.243584285714286)
		(4.93,0.247347142857143)
		(4.94,0.250988619047619)
		(4.95,0.254508714285714)
		(4.96,0.25815019047619)
		(4.97,0.261548904761905)
		(4.98,0.264462095238095)
		(4.99,0.266889714285714)
		(5,0.269195952380952)
		(5.01,0.270773904761905)
		(5.02,0.272230476190476)
		(5.03,0.274172571428571)
		(5.04,0.275386380952381)
		(5.05,0.276842952380952)
		(5.06,0.278663666666667)
		(5.07,0.280484380952381)
		(5.08,0.282183714285714)
		(5.09,0.284732761904762)
		(5.1,0.287039047619048)
		(5.11,0.288859809523809)
		(5.12,0.290437761904762)
		(5.13,0.291773)
		(5.14,0.292744047619048)
		(5.15,0.293472380952381)
		(5.16,0.294322047619048)
		(5.17,0.294807571428571)
		(5.18,0.295293095238095)
		(5.19,0.295535857142857)
		(5.2,0.296021380952381)
		(5.21,0.296385523809524)
		(5.22,0.297478)
		(5.23,0.298570476190476)
		(5.24,0.29942019047619)
		(5.25,0.300755428571429)
		(5.26,0.301726523809524)
		(5.27,0.303183142857143)
		(5.28,0.303911476190476)
		(5.29,0.305125333333333)
		(5.3,0.305853619047619)
		(5.31,0.305853619047619)
		(5.32,0.306460523809524)
		(5.33,0.306703333333333)
		(5.34,0.307188857142857)
		(5.35,0.30779580952381)
		(5.36,0.308281333333333)
		(5.37,0.308159952380952)
		(5.38,0.30791719047619)
		(5.39,0.308281380952381)
		(5.4,0.308281380952381)
		(5.41,0.30816)
		(5.42,0.308281380952381)
		(5.43,0.307310285714286)
		(5.44,0.306581952380952)
		(5.45,0.305489476190476)
		(5.46,0.304761142857143)
		(5.47,0.303790047619048)
		(5.48,0.30245480952381)
		(5.49,0.301605095238095)
		(5.5,0.299905714285714)
		(5.51,0.298570476190476)
		(5.52,0.297356619047619)
		(5.53,0.295535857142857)
		(5.54,0.294443380952381)
		(5.55,0.292379857142857)
		(5.56,0.290437714285714)
		(5.57,0.288616952380952)
		(5.58,0.287281761904762)
		(5.59,0.285946571428571)
		(5.6,0.284004428571429)
		(5.61,0.282790619047619)
		(5.62,0.280969904761905)
		(5.63,0.279391952380952)
		(5.64,0.278299523809524)
		(5.65,0.276236047619048)
		(5.66,0.274658095238095)
		(5.67,0.272351857142857)
		(5.68,0.270409761904762)
		(5.69,0.268589047619048)
		(5.7,0.266404190476191)
		(5.71,0.265069)
		(5.72,0.262641380952381)
		(5.73,0.260577904761905)
		(5.74,0.258878571428571)
		(5.75,0.257057857142857)
		(5.76,0.255965428571429)
		(5.77,0.254873)
		(5.78,0.253052285714286)
		(5.79,0.252081238095238)
		(5.8,0.251231571428571)
		(5.81,0.249896380952381)
		(5.82,0.248803952380952)
		(5.83,0.247711523809524)
		(5.84,0.246497714285714)
		(5.85,0.245162523809524)
		(5.86,0.244798380952381)
		(5.87,0.243948714285714)
		(5.88,0.243341809523809)
		(5.89,0.243099047619048)
		(5.9,0.242128)
		(5.91,0.241156904761905)
		(5.92,0.240428619047619)
		(5.93,0.240064476190476)
		(5.94,0.240064476190476)
		(5.95,0.239578952380952)
		(5.96,0.238972047619048)
		(5.97,0.238122380952381)
		(5.98,0.237272666666667)
		(5.99,0.236908476190476)
		(6,0.236058761904762)
		(6.01,0.235087666666667)
		(6.02,0.234602095238095)
		(6.03,0.233995142857143)
		(6.04,0.233995142857143)
		(6.05,0.23326680952381)
		(6.06,0.232781238095238)
		(6.07,0.232052904761905)
		(6.08,0.231324571428571)
		(6.09,0.230717619047619)
		(6.1,0.229867904761905)
		(6.11,0.22901819047619)
		(6.12,0.228896809523809)
		(6.13,0.228411238095238)
		(6.14,0.227925666666667)
		(6.15,0.227197333333333)
		(6.16,0.226590380952381)
		(6.17,0.22610480952381)
		(6.18,0.225619238095238)
		(6.19,0.225255095238095)
		(6.2,0.225133714285714)
		(6.21,0.22452680952381)
		(6.22,0.224284047619048)
		(6.23,0.223919904761905)
		(6.24,0.223555761904762)
		(6.25,0.222584666666667)
		(6.26,0.222099142857143)
		(6.27,0.221613619047619)
		(6.28,0.221249476190476)
		(6.29,0.221370857142857)
		(6.3,0.221370857142857)
		(6.31,0.221370857142857)
		(6.32,0.221735)
		(6.33,0.221370857142857)
		(6.34,0.220763952380952)
		(6.35,0.220642571428571)
		(6.36,0.220278428571429)
		(6.37,0.219550142857143)
		(6.38,0.219307380952381)
		(6.39,0.218943238095238)
		(6.4,0.218821857142857)
		(6.41,0.218214952380952)
		(6.42,0.217729428571429)
		(6.43,0.217001142857143)
		(6.44,0.216758380952381)
		(6.45,0.216272857142857)
		(6.46,0.216272857142857)
		(6.47,0.216272857142857)
		(6.48,0.216272857142857)
		(6.49,0.216030095238095)
		(6.5,0.21542319047619)
		(6.51,0.214452142857143)
		(6.52,0.214209380952381)
		(6.53,0.213845238095238)
		(6.54,0.213481095238095)
		(6.55,0.21287419047619)
		(6.56,0.212267285714286)
		(6.57,0.212145904761905)
		(6.58,0.212145904761905)
		(6.59,0.211539)
		(6.6,0.211296238095238)
		(6.61,0.210810714285714)
		(6.62,0.210567952380952)
		(6.63,0.210932095238095)
		(6.64,0.211296238095238)
		(6.65,0.211053476190476)
		(6.66,0.210810714285714)
		(6.67,0.210203809523809)
		(6.68,0.209718285714286)
		(6.69,0.209111380952381)
		(6.7,0.208747238095238)
		(6.71,0.208747238095238)
		(6.72,0.208868619047619)
		(6.73,0.208140333333333)
		(6.74,0.207897571428571)
		(6.75,0.207776190476191)
		(6.76,0.207897571428571)
		(6.77,0.207776190476191)
		(6.78,0.207412047619048)
		(6.79,0.207533428571429)
		(6.8,0.207412047619048)
		(6.81,0.207290666666667)
		(6.82,0.206926523809524)
		(6.83,0.206805142857143)
		(6.84,0.206683761904762)
		(6.85,0.206319619047619)
		(6.86,0.205834095238095)
		(6.87,0.205591333333333)
		(6.88,0.206198238095238)
		(6.89,0.206441)
		(6.9,0.206441)
		(6.91,0.206319619047619)
		(6.92,0.205591333333333)
		(6.93,0.205348571428571)
		(6.94,0.20510580952381)
		(6.95,0.204620285714286)
		(6.96,0.204256142857143)
		(6.97,0.203892)
		(6.98,0.203527857142857)
		(6.99,0.203042333333333)
		(7,0.20267819047619)
		(7.01,0.203042333333333)
		(7.02,0.202920952380952)
		(7.03,0.203042333333333)
		(7.04,0.202920952380952)
		(7.05,0.202435428571429)
		(7.06,0.202192666666667)
		(7.07,0.20267819047619)
		(7.08,0.203042333333333)
		(7.09,0.202192666666667)
		(7.1,0.201585761904762)
		(7.11,0.201221619047619)
		(7.12,0.200857476190476)
		(7.13,0.201100238095238)
		(7.14,0.201343)
		(7.15,0.201707142857143)
		(7.16,0.201949904761905)
		(7.17,0.202435428571429)
		(7.18,0.20255680952381)
		(7.19,0.20267819047619)
		(7.2,0.202920952380952)
		(7.21,0.202799571428571)
		(7.22,0.202799571428571)
		(7.23,0.202314047619048)
		(7.24,0.20255680952381)
		(7.25,0.20267819047619)
		(7.26,0.202314047619048)
		(7.27,0.202314047619048)
		(7.28,0.201707142857143)
		(7.29,0.201221619047619)
		(7.3,0.201707142857143)
		(7.31,0.201949904761905)
		(7.32,0.202435428571429)
		(7.33,0.202678190476191)
		(7.34,0.202920952380952)
		(7.35,0.202678190476191)
		(7.36,0.202435428571429)
		(7.37,0.202435428571429)
		(7.38,0.201949904761905)
		(7.39,0.201585761904762)
		(7.4,0.201464380952381)
		(7.41,0.201585761904762)
		(7.42,0.201221619047619)
		(7.43,0.200857476190476)
		(7.44,0.201221619047619)
		(7.45,0.200857476190476)
		(7.46,0.200493333333333)
		(7.47,0.201100238095238)
		(7.48,0.200736095238095)
		(7.49,0.200857476190476)
		(7.5,0.201343)
		(7.51,0.200736095238095)
		(7.52,0.200614714285714)
		(7.53,0.200250571428571)
		(7.54,0.200250571428571)
		(7.55,0.200250571428571)
		(7.56,0.199765047619048)
		(7.57,0.199886428571429)
		(7.58,0.199643666666667)
		(7.59,0.199643666666667)
		(7.6,0.200007809523809)
		(7.61,0.20012919047619)
		(7.62,0.200007809523809)
		(7.63,0.20000780952381)
		(7.64,0.20012919047619)
		(7.65,0.199886428571429)
		(7.66,0.199643666666667)
		(7.67,0.199643666666667)
		(7.68,0.199279523809524)
		(7.69,0.199765047619048)
		(7.7,0.199522285714286)
		(7.71,0.199036761904762)
		(7.72,0.199158142857143)
		(7.73,0.199158142857143)
		(7.74,0.199036761904762)
		(7.75,0.198551238095238)
		(7.76,0.198429857142857)
		(7.77,0.198429857142857)
		(7.78,0.198429857142857)
		(7.79,0.198308476190476)
		(7.8,0.198187095238095)
		(7.81,0.197944333333333)
		(7.82,0.197944333333333)
		(7.83,0.197458809523809)
		(7.84,0.197701571428571)
		(7.85,0.197337428571429)
		(7.86,0.19758019047619)
		(7.87,0.197337428571429)
		(7.88,0.197216047619048)
		(7.89,0.196851904761905)
		(7.9,0.196730523809524)
		(7.91,0.196609142857143)
		(7.92,0.196609142857143)
		(7.93,0.196609142857143)
		(7.94,0.196487761904762)
		(7.95,0.196123619047619)
		(7.96,0.196366380952381)
		(7.97,0.195638095238095)
		(7.98,0.195638095238095)
		(7.99,0.195273952380952)
		(8,0.194909809523809)
		(8.01,0.195152571428571)
		(8.02,0.195516714285714)
		(8.03,0.195273952380952)
		(8.04,0.195152571428571)
		(8.05,0.19490980952381)
		(8.06,0.194788428571429)
		(8.07,0.194788428571429)
		(8.08,0.19503119047619)
		(8.09,0.194667047619048)
		(8.1,0.194788428571429)
		(8.11,0.194181523809524)
		(8.12,0.194788428571429)
		(8.13,0.194788428571429)
		(8.14,0.195152571428571)
		(8.15,0.195152571428571)
		(8.16,0.195880857142857)
		(8.17,0.195880857142857)
		(8.18,0.196245)
		(8.19,0.196487761904762)
		(8.2,0.196366380952381)
		(8.21,0.196851904761905)
		(8.22,0.196487761904762)
		(8.23,0.196002238095238)
		(8.24,0.195880857142857)
		(8.25,0.196245)
		(8.26,0.196002238095238)
		(8.27,0.196123619047619)
		(8.28,0.195759476190476)
		(8.29,0.195638095238095)
		(8.3,0.196002238095238)
		(8.31,0.195638095238095)
		(8.32,0.195880857142857)
		(8.33,0.195516714285714)
		(8.34,0.195152571428571)
		(8.35,0.194667047619048)
		(8.36,0.194545666666667)
		(8.37,0.194181523809524)
		(8.38,0.194060142857143)
		(8.39,0.194060142857143)
		(8.4,0.193938761904762)
		(8.41,0.193938761904762)
		(8.42,0.193817380952381)
		(8.43,0.193574619047619)
		(8.44,0.193574619047619)
		(8.45,0.193817380952381)
		(8.46,0.193696)
		(8.47,0.193938761904762)
		(8.48,0.193817380952381)
		(8.49,0.193453238095238)
		(8.5,0.193453238095238)
		(8.51,0.193696)
		(8.52,0.193817380952381)
		(8.53,0.193696)
		(8.54,0.193453238095238)
		(8.55,0.193331857142857)
		(8.56,0.193331857142857)
		(8.57,0.193210476190476)
		(8.58,0.192846333333333)
		(8.59,0.192846333333333)
		(8.6,0.192360809523809)
		(8.61,0.192360809523809)
		(8.62,0.192118047619048)
		(8.63,0.191996666666667)
		(8.64,0.191996666666667)
		(8.65,0.192239428571429)
		(8.66,0.191632523809524)
		(8.67,0.191511142857143)
		(8.68,0.191511142857143)
		(8.69,0.191511142857143)
		(8.7,0.191511142857143)
		(8.71,0.191147)
		(8.72,0.191147)
		(8.73,0.191147)
		(8.74,0.191268380952381)
		(8.75,0.191025619047619)
		(8.76,0.191268380952381)
		(8.77,0.191268380952381)
		(8.78,0.191025619047619)
		(8.79,0.190904238095238)
		(8.8,0.190782857142857)
		(8.81,0.191389761904762)
		(8.82,0.191025619047619)
		(8.83,0.191147)
		(8.84,0.190661476190476)
		(8.85,0.190661476190476)
		(8.86,0.190540095238095)
		(8.87,0.190782857142857)
		(8.88,0.190418714285714)
		(8.89,0.190540095238095)
		(8.9,0.190661476190476)
		(8.91,0.191025619047619)
		(8.92,0.191511142857143)
		(8.93,0.191147)
		(8.94,0.191268380952381)
		(8.95,0.191268380952381)
		(8.96,0.191147)
		(8.97,0.191268380952381)
		(8.98,0.190904238095238)
		(8.99,0.190782857142857)
		};

==> addplot__Dilution75.tex <==
\addplot [black, thick] coordinates{
		(0,0.330494333333333)
		(0.01,0.330858476190476)
		(0.02,0.330858476190476)
		(0.03,0.330858476190476)
		(0.04,0.330858476190476)
		(0.05,0.331101238095238)
		(0.06,0.331465380952381)
		(0.07,0.330979857142857)
		(0.08,0.330979857142857)
		(0.09,0.330858476190476)
		(0.1,0.330737095238095)
		(0.11,0.331344)
		(0.12,0.331586761904762)
		(0.13,0.331344)
		(0.14,0.330737095238095)
		(0.15,0.330737095238095)
		(0.16,0.330615714285714)
		(0.17,0.330494333333333)
		(0.18,0.330494333333333)
		(0.19,0.330858476190476)
		(0.2,0.330130190476191)
		(0.21,0.330372952380952)
		(0.22,0.329766047619048)
		(0.23,0.329523285714286)
		(0.24,0.329401904761905)
		(0.25,0.329401904761905)
		(0.26,0.329523285714286)
		(0.27,0.329280523809524)
		(0.28,0.329159142857143)
		(0.29,0.328552238095238)
		(0.3,0.328430857142857)
		(0.31,0.328673619047619)
		(0.32,0.328066714285714)
		(0.33,0.327945333333333)
		(0.34,0.328188095238095)
		(0.35,0.328673619047619)
		(0.36,0.328309476190476)
		(0.37,0.328309476190476)
		(0.38,0.328309476190476)
		(0.39,0.328188095238095)
		(0.4,0.32758119047619)
		(0.41,0.327945333333333)
		(0.42,0.327702571428571)
		(0.43,0.328188095238095)
		(0.44,0.328795)
		(0.45,0.329159142857143)
		(0.46,0.329159142857143)
		(0.47,0.328430857142857)
		(0.48,0.328066714285714)
		(0.49,0.328309476190476)
		(0.5,0.328795)
		(0.51,0.329159142857143)
		(0.52,0.329159142857143)
		(0.53,0.329280523809524)
		(0.54,0.329159142857143)
		(0.55,0.329159142857143)
		(0.56,0.328673619047619)
		(0.57,0.328430857142857)
		(0.58,0.327945333333333)
		(0.59,0.32745980952381)
		(0.6,0.327338428571429)
		(0.61,0.327338428571428)
		(0.62,0.327338428571429)
		(0.63,0.327338428571429)
		(0.64,0.32745980952381)
		(0.65,0.327217047619048)
		(0.66,0.32745980952381)
		(0.67,0.327823952380952)
		(0.68,0.328066714285714)
		(0.69,0.328066714285714)
		(0.7,0.328066714285714)
		(0.71,0.328188095238095)
		(0.72,0.328066714285714)
		(0.73,0.328309476190476)
		(0.74,0.328552238095238)
		(0.75,0.329280523809524)
		(0.76,0.329523285714286)
		(0.77,0.330251571428572)
		(0.78,0.331101238095238)
		(0.79,0.333043333333333)
		(0.8,0.334742666666667)
		(0.81,0.336442)
		(0.82,0.338384095238095)
		(0.83,0.340204809523809)
		(0.84,0.342268285714286)
		(0.85,0.344210428571429)
		(0.86,0.346516714285714)
		(0.87,0.348944380952381)
		(0.88,0.351372047619048)
		(0.89,0.354649380952381)
		(0.9,0.358169476190476)
		(0.91,0.362053714285714)
		(0.92,0.365937952380952)
		(0.93,0.370307714285714)
		(0.94,0.374070571428571)
		(0.95,0.37807619047619)
		(0.96,0.381717666666667)
		(0.97,0.385844666666667)
		(0.98,0.389607523809524)
		(0.99,0.393127619047619)
		(1,0.396526333333333)
		(1.01,0.399925047619048)
		(1.02,0.402716857142857)
		(1.03,0.405630047619048)
		(1.04,0.408543238095238)
		(1.05,0.411820571428571)
		(1.06,0.415219238095238)
		(1.07,0.418375142857143)
		(1.08,0.421531095238095)
		(1.09,0.424565666666667)
		(1.1,0.426871904761905)
		(1.11,0.429178142857143)
		(1.12,0.430149190476191)
		(1.13,0.430998857142857)
		(1.14,0.431969904761905)
		(1.15,0.433062333333333)
		(1.16,0.433912)
		(1.17,0.43512580952381)
		(1.18,0.436582428571429)
		(1.19,0.438039)
		(1.2,0.439495571428571)
		(1.21,0.440709428571429)
		(1.22,0.441923285714286)
		(1.23,0.443744047619048)
		(1.24,0.44568619047619)
		(1.25,0.447749714285714)
		(1.26,0.44884219047619)
		(1.27,0.449327761904762)
		(1.28,0.449691952380952)
		(1.29,0.450056095238095)
		(1.3,0.450541619047619)
		(1.31,0.451148571428571)
		(1.32,0.451634142857143)
		(1.33,0.452848)
		(1.34,0.454061857142857)
		(1.35,0.45466880952381)
		(1.36,0.455761285714286)
		(1.37,0.456853761904762)
		(1.38,0.457096523809524)
		(1.39,0.456732333333333)
		(1.4,0.456368190476191)
		(1.41,0.45624680952381)
		(1.42,0.455639857142857)
		(1.43,0.454790142857143)
		(1.44,0.454304571428572)
		(1.45,0.453333476190476)
		(1.46,0.451755476190476)
		(1.47,0.451269952380952)
		(1.48,0.450663)
		(1.49,0.450541619047619)
		(1.5,0.450056047619048)
		(1.51,0.449449095238095)
		(1.52,0.449449095238095)
		(1.53,0.448963523809524)
		(1.54,0.448477952380952)
		(1.55,0.447749619047619)
		(1.56,0.446535761904762)
		(1.57,0.445079142857143)
		(1.58,0.443622523809524)
		(1.59,0.442287333333333)
		(1.6,0.441437666666667)
		(1.61,0.439981095238095)
		(1.62,0.439010047619048)
		(1.63,0.437432095238095)
		(1.64,0.436218285714286)
		(1.65,0.435004476190476)
		(1.66,0.433426523809524)
		(1.67,0.431848571428571)
		(1.68,0.429299523809524)
		(1.69,0.427600190476191)
		(1.7,0.425172523809524)
		(1.71,0.422866285714286)
		(1.72,0.420560047619048)
		(1.73,0.417404095238095)
		(1.74,0.414855095238095)
		(1.75,0.412306095238095)
		(1.76,0.409392952380952)
		(1.77,0.407450857142857)
		(1.78,0.405630142857143)
		(1.79,0.404294952380952)
		(1.8,0.402838380952381)
		(1.81,0.401139047619048)
		(1.82,0.400046619047619)
		(1.83,0.398225904761905)
		(1.84,0.396647952380952)
		(1.85,0.39507)
		(1.86,0.393249285714286)
		(1.87,0.391307142857143)
		(1.88,0.389607761904762)
		(1.89,0.388758095238095)
		(1.9,0.387058714285714)
		(1.91,0.385602095238095)
		(1.92,0.384266857142857)
		(1.93,0.383174428571428)
		(1.94,0.382081952380952)
		(1.95,0.381475047619047)
		(1.96,0.380503952380952)
		(1.97,0.379897)
		(1.98,0.378925904761905)
		(1.99,0.377954809523809)
		(2,0.37649819047619)
		(2.01,0.375284333333333)
		(2.02,0.374313238095238)
		(2.03,0.373584904761905)
		(2.04,0.372249666666667)
		(2.05,0.371764095238095)
		(2.06,0.370914380952381)
		(2.07,0.370428809523809)
		(2.08,0.370186047619048)
		(2.09,0.369943285714286)
		(2.1,0.369093571428571)
		(2.11,0.368365285714286)
		(2.12,0.368365285714286)
		(2.13,0.368001142857143)
		(2.14,0.367030047619048)
		(2.15,0.366787285714286)
		(2.16,0.365937571428571)
		(2.17,0.365330666666667)
		(2.18,0.364723761904762)
		(2.19,0.364238238095238)
		(2.2,0.363509952380952)
		(2.21,0.363024428571429)
		(2.22,0.362781666666667)
		(2.23,0.362296142857143)
		(2.24,0.361567857142857)
		(2.25,0.361932)
		(2.26,0.361567857142857)
		(2.27,0.361082333333333)
		(2.28,0.359989904761905)
		(2.29,0.359504380952381)
		(2.3,0.359018857142857)
		(2.31,0.358533333333333)
		(2.32,0.358290571428571)
		(2.33,0.357562285714286)
		(2.34,0.356712619047619)
		(2.35,0.356348476190476)
		(2.36,0.355620190476191)
		(2.37,0.35549880952381)
		(2.38,0.354891904761905)
		(2.39,0.354649142857143)
		(2.4,0.354649142857143)
		(2.41,0.354527761904762)
		(2.42,0.354163619047619)
		(2.43,0.353435333333333)
		(2.44,0.353313952380952)
		(2.45,0.352828428571429)
		(2.46,0.352342904761905)
		(2.47,0.351614619047619)
		(2.48,0.351371857142857)
		(2.49,0.351371857142857)
		(2.5,0.351007714285714)
		(2.51,0.350764952380952)
		(2.52,0.35052219047619)
		(2.53,0.35052219047619)
		(2.54,0.350279428571429)
		(2.55,0.350764952380952)
		(2.56,0.350643571428571)
		(2.57,0.35052219047619)
		(2.58,0.349793904761905)
		(2.59,0.349551142857143)
		(2.6,0.348944238095238)
		(2.61,0.348215952380952)
		(2.62,0.34785180952381)
		(2.63,0.347609047619048)
		(2.64,0.347609047619048)
		(2.65,0.347123523809524)
		(2.66,0.347002142857143)
		(2.67,0.346516619047619)
		(2.68,0.346516619047619)
		(2.69,0.346395238095238)
		(2.7,0.346152476190476)
		(2.71,0.345788333333333)
		(2.72,0.345302809523809)
		(2.73,0.345060047619048)
		(2.74,0.344695904761905)
		(2.75,0.344695904761905)
		(2.76,0.344817285714286)
		(2.77,0.346031095238095)
		(2.78,0.347609095238095)
		(2.79,0.349672619047619)
		(2.8,0.352464428571429)
		(2.81,0.355377619047619)
		(2.82,0.35841219047619)
		(2.83,0.362053666666667)
		(2.84,0.365573761904762)
		(2.85,0.369458)
		(2.86,0.373220857142857)
		(2.87,0.377226476190476)
		(2.88,0.380867952380952)
		(2.89,0.384388047619048)
		(2.9,0.388150904761905)
		(2.91,0.391792380952381)
		(2.92,0.395312476190476)
		(2.93,0.399075333333333)
		(2.94,0.402959571428571)
		(2.95,0.406843809523809)
		(2.96,0.410606666666667)
		(2.97,0.413762619047619)
		(2.98,0.416433047619048)
		(2.99,0.418982047619048)
		(3,0.421288285714286)
		(3.01,0.423715952380952)
		(3.02,0.425536666666667)
		(3.03,0.42760019047619)
		(3.04,0.428935380952381)
		(3.05,0.430149190476191)
		(3.06,0.430998857142857)
		(3.07,0.431848523809524)
		(3.08,0.432455428571429)
		(3.09,0.433547857142857)
		(3.1,0.434518904761905)
		(3.11,0.435368571428571)
		(3.12,0.436339619047619)
		(3.13,0.437917571428571)
		(3.14,0.439616952380952)
		(3.15,0.441073571428571)
		(3.16,0.442651571428571)
		(3.17,0.444715095238095)
		(3.18,0.4469)
		(3.19,0.448599380952381)
		(3.2,0.449934619047619)
		(3.21,0.451512619047619)
		(3.22,0.451876761904762)
		(3.23,0.452483714285714)
		(3.24,0.452483714285714)
		(3.25,0.452483714285714)
		(3.26,0.452969285714286)
		(3.27,0.453090666666667)
		(3.28,0.453454857142857)
		(3.29,0.453819)
		(3.3,0.45418319047619)
		(3.31,0.455032904761905)
		(3.32,0.455518476190476)
		(3.33,0.456004047619048)
		(3.34,0.456004047619048)
		(3.35,0.456125428571429)
		(3.36,0.455882666666667)
		(3.37,0.455761285714286)
		(3.38,0.455518523809524)
		(3.39,0.454911619047619)
		(3.4,0.454547476190476)
		(3.41,0.454547476190476)
		(3.42,0.45381919047619)
		(3.43,0.45381919047619)
		(3.44,0.453940571428571)
		(3.45,0.454304714285714)
		(3.46,0.454911666666667)
		(3.47,0.455154428571429)
		(3.48,0.45564)
		(3.49,0.45564)
		(3.5,0.455033095238095)
		(3.51,0.454062)
		(3.52,0.452362619047619)
		(3.53,0.450906)
		(3.54,0.448963857142857)
		(3.55,0.447143142857143)
		(3.56,0.445079619047619)
		(3.57,0.442894714285714)
		(3.58,0.44070980952381)
		(3.59,0.438403523809524)
		(3.6,0.436461380952381)
		(3.61,0.434640619047619)
		(3.62,0.432334333333333)
		(3.63,0.430149428571429)
		(3.64,0.427721761904762)
		(3.65,0.425172714285714)
		(3.66,0.422380904761905)
		(3.67,0.419589095238095)
		(3.68,0.416918666666667)
		(3.69,0.414733761904762)
		(3.7,0.412306095238095)
		(3.71,0.410970904761905)
		(3.72,0.409392952380952)
		(3.73,0.408421904761905)
		(3.74,0.407450857142857)
		(3.75,0.406601190476191)
		(3.76,0.405994285714286)
		(3.77,0.405266)
		(3.78,0.404780476190476)
		(3.79,0.403566666666667)
		(3.8,0.402231476190476)
		(3.81,0.400896285714286)
		(3.82,0.399803857142857)
		(3.83,0.399075571428571)
		(3.84,0.398347285714286)
		(3.85,0.397254857142857)
		(3.86,0.396041047619048)
		(3.87,0.395434142857143)
		(3.88,0.394584476190476)
		(3.89,0.393977571428571)
		(3.9,0.393006523809524)
		(3.91,0.392156857142857)
		(3.92,0.390943047619048)
		(3.93,0.390093380952381)
		(3.94,0.389122333333333)
		(3.95,0.387787095238095)
		(3.96,0.386694619047619)
		(3.97,0.385602142857143)
		(3.98,0.384388285714286)
		(3.99,0.383295809523809)
		(4,0.382810285714286)
		(4.01,0.382324761904762)
		(4.02,0.381232285714286)
		(4.03,0.379897047619047)
		(4.04,0.378561809523809)
		(4.05,0.377347952380952)
		(4.06,0.376619619047619)
		(4.07,0.376134047619048)
		(4.08,0.375041571428571)
		(4.09,0.374313238095238)
		(4.1,0.373220761904762)
		(4.11,0.372249666666667)
		(4.12,0.371521333333333)
		(4.13,0.370428857142857)
		(4.14,0.369457761904762)
		(4.15,0.368850809523809)
		(4.16,0.368243904761905)
		(4.17,0.368122523809524)
		(4.18,0.367879761904762)
		(4.19,0.367515619047619)
		(4.2,0.367394238095238)
		(4.21,0.366423142857143)
		(4.22,0.365694809523809)
		(4.23,0.36569480952381)
		(4.24,0.365452047619048)
		(4.25,0.365209285714286)
		(4.26,0.364845142857143)
		(4.27,0.364602380952381)
		(4.28,0.364238238095238)
		(4.29,0.363995476190476)
		(4.3,0.363145809523809)
		(4.31,0.362538904761905)
		(4.32,0.361932)
		(4.33,0.361567857142857)
		(4.34,0.361446476190476)
		(4.35,0.361446476190476)
		(4.36,0.361325095238095)
		(4.37,0.361567857142857)
		(4.38,0.361325095238095)
		(4.39,0.36071819047619)
		(4.4,0.360475428571429)
		(4.41,0.360111285714286)
		(4.42,0.360232666666667)
		(4.43,0.360111285714286)
		(4.44,0.359747142857143)
		(4.45,0.359383)
		(4.46,0.359261619047619)
		(4.47,0.359140238095238)
		(4.48,0.358897476190476)
		(4.49,0.359018857142857)
		(4.5,0.358897476190476)
		(4.51,0.358897476190476)
		(4.52,0.358776095238095)
		(4.53,0.358654714285714)
		(4.54,0.358290571428572)
		(4.55,0.358290571428572)
		(4.56,0.357926428571429)
		(4.57,0.356955380952381)
		(4.58,0.355984333333333)
		(4.59,0.355134666666667)
		(4.6,0.354649142857143)
		(4.61,0.354042238095238)
		(4.62,0.353678095238095)
		(4.63,0.353313952380952)
		(4.64,0.352828428571429)
		(4.65,0.352221523809524)
		(4.66,0.352100142857143)
		(4.67,0.351736)
		(4.68,0.351250476190476)
		(4.69,0.35052219047619)
		(4.7,0.349915285714286)
		(4.71,0.349429761904762)
		(4.72,0.349187)
		(4.73,0.348822857142857)
		(4.74,0.348580095238095)
		(4.75,0.348580095238095)
		(4.76,0.348215952380952)
		(4.77,0.348580095238095)
		(4.78,0.349551142857143)
		(4.79,0.350764952380952)
		(4.8,0.351978761904762)
		(4.81,0.353556761904762)
		(4.82,0.355741666666667)
		(4.83,0.357319666666667)
		(4.84,0.359019047619048)
		(4.85,0.361082571428571)
		(4.86,0.363510238095238)
		(4.87,0.365331)
		(4.88,0.367880047619048)
		(4.89,0.370307714285714)
		(4.9,0.373706428571429)
		(4.91,0.376619619047619)
		(4.92,0.380018333333333)
		(4.93,0.383417047619048)
		(4.94,0.38778680952381)
		(4.95,0.391792428571429)
		(4.96,0.396526380952381)
		(4.97,0.401260285714286)
		(4.98,0.405630095238095)
		(4.99,0.409635714285714)
		(5,0.413155809523809)
		(5.01,0.417040095238095)
		(5.02,0.420196)
		(5.03,0.422745)
		(5.04,0.425294)
		(5.05,0.427721619047619)
		(5.06,0.429906476190476)
		(5.07,0.432576904761905)
		(5.08,0.435732857142857)
		(5.09,0.438403285714286)
		(5.1,0.441559238095238)
		(5.11,0.443986904761905)
		(5.12,0.446535952380952)
		(5.13,0.448720857142857)
		(5.14,0.450420238095238)
		(5.15,0.451512714285714)
		(5.16,0.452847952380952)
		(5.17,0.452847952380952)
		(5.18,0.452726571428571)
		(5.19,0.452726571428571)
		(5.2,0.452848)
		(5.21,0.453333571428571)
		(5.22,0.453697714285714)
		(5.23,0.453819095238095)
		(5.24,0.454061904761905)
		(5.25,0.455154380952381)
		(5.26,0.456125476190476)
		(5.27,0.45697519047619)
		(5.28,0.457217952380952)
		(5.29,0.457824857142857)
		(5.3,0.457824857142857)
		(5.31,0.457946238095238)
		(5.32,0.458189)
		(5.33,0.458553142857143)
		(5.34,0.458795904761905)
		(5.35,0.45940280952381)
		(5.36,0.459766952380952)
		(5.37,0.459888333333333)
		(5.38,0.460859380952381)
		(5.39,0.461709095238095)
		(5.4,0.462680142857143)
		(5.41,0.463408428571429)
		(5.42,0.463893952380952)
		(5.43,0.464015333333333)
		(5.44,0.464136761904762)
		(5.45,0.464015333333333)
		(5.46,0.463287)
		(5.47,0.462922857142857)
		(5.48,0.462194523809524)
		(5.49,0.461223428571429)
		(5.5,0.45976680952381)
		(5.51,0.458674333333334)
		(5.52,0.457339095238095)
		(5.53,0.455761095238095)
		(5.54,0.454790047619048)
		(5.55,0.453697571428572)
		(5.56,0.452847857142857)
		(5.57,0.451876761904762)
		(5.58,0.451027047619048)
		(5.59,0.44969180952381)
		(5.6,0.448477952380952)
		(5.61,0.446657190476191)
		(5.62,0.444715047619048)
		(5.63,0.442772904761905)
		(5.64,0.441073523809524)
		(5.65,0.439616904761905)
		(5.66,0.438038952380952)
		(5.67,0.436582380952381)
		(5.68,0.435125761904762)
		(5.69,0.43354780952381)
		(5.7,0.432212619047619)
		(5.71,0.43112019047619)
		(5.72,0.429906380952381)
		(5.73,0.428571190476191)
		(5.74,0.427236)
		(5.75,0.424929714285714)
		(5.76,0.422866238095238)
		(5.77,0.420681380952381)
		(5.78,0.418375142857143)
		(5.79,0.416068904761905)
		(5.8,0.413519904761905)
		(5.81,0.411213666666667)
		(5.82,0.409392952380952)
		(5.83,0.408179142857143)
		(5.84,0.406843952380952)
		(5.85,0.405266)
		(5.86,0.40393080952381)
		(5.87,0.402474238095238)
		(5.88,0.400774904761905)
		(5.89,0.399075571428571)
		(5.9,0.397861761904762)
		(5.91,0.39628380952381)
		(5.92,0.394584476190476)
		(5.93,0.393127904761905)
		(5.94,0.391792714285714)
		(5.95,0.390578904761905)
		(5.96,0.389486476190476)
		(5.97,0.388515428571428)
		(5.98,0.38718019047619)
		(5.99,0.386087714285714)
		(6,0.385116666666667)
		(6.01,0.384388333333333)
		(6.02,0.383902809523809)
		(6.03,0.383174523809524)
		(6.04,0.382082095238095)
		(6.05,0.380868238095238)
		(6.06,0.379897142857143)
		(6.07,0.379047428571429)
		(6.08,0.378197714285714)
		(6.09,0.377469380952381)
		(6.1,0.376862428571429)
		(6.11,0.375891333333333)
		(6.12,0.375284380952381)
		(6.13,0.374313285714286)
		(6.14,0.37322080952381)
		(6.15,0.372371095238095)
		(6.16,0.371278619047619)
		(6.17,0.370550285714286)
		(6.18,0.369700571428571)
		(6.19,0.369215047619048)
		(6.2,0.368608142857143)
		(6.21,0.368122571428571)
		(6.22,0.367637047619048)
		(6.23,0.366908714285714)
		(6.24,0.365937619047619)
		(6.25,0.364723761904762)
		(6.26,0.364359619047619)
		(6.27,0.363995476190476)
		(6.28,0.36326719047619)
		(6.29,0.362538904761905)
		(6.3,0.361810619047619)
		(6.31,0.361203714285714)
		(6.32,0.36059680952381)
		(6.33,0.360354047619048)
		(6.34,0.360232666666667)
		(6.35,0.359747142857143)
		(6.36,0.359018857142857)
		(6.37,0.359018857142857)
		(6.38,0.358654714285714)
		(6.39,0.358169190476191)
		(6.4,0.357440904761905)
		(6.41,0.356712619047619)
		(6.42,0.356105714285714)
		(6.43,0.355377428571429)
		(6.44,0.354770523809524)
		(6.45,0.354406380952381)
		(6.46,0.354770523809524)
		(6.47,0.354406380952381)
		(6.48,0.353435333333333)
		(6.49,0.35294980952381)
		(6.5,0.352585666666667)
		(6.51,0.352221523809524)
		(6.52,0.351493238095238)
		(6.53,0.351250476190476)
		(6.54,0.351007714285714)
		(6.55,0.351007714285714)
		(6.56,0.351371857142857)
		(6.57,0.351129095238095)
		(6.58,0.35040080952381)
		(6.59,0.350036666666667)
		(6.6,0.349793904761905)
		(6.61,0.349793904761905)
		(6.62,0.349551142857143)
		(6.63,0.348944238095238)
		(6.64,0.348822857142857)
		(6.65,0.348337333333333)
		(6.66,0.347730428571429)
		(6.67,0.346880761904762)
		(6.68,0.346395238095238)
		(6.69,0.346395238095238)
		(6.7,0.346516619047619)
		(6.71,0.346273857142857)
		(6.72,0.346395238095238)
		(6.73,0.346516619047619)
		(6.74,0.346395238095238)
		(6.75,0.346273857142857)
		(6.76,0.34542419047619)
		(6.77,0.344574523809524)
		(6.78,0.344574523809524)
		(6.79,0.344453142857143)
		(6.8,0.344210380952381)
		(6.81,0.343603476190476)
		(6.82,0.343603476190476)
		(6.83,0.343724857142857)
		(6.84,0.343603476190476)
		(6.85,0.343603476190476)
		(6.86,0.343360714285714)
		(6.87,0.343603476190476)
		(6.88,0.343967619047619)
		(6.89,0.343603476190476)
		(6.9,0.343239333333333)
		(6.91,0.343117952380952)
		(6.92,0.343603476190476)
		(6.93,0.343482095238095)
		(6.94,0.342996571428571)
		(6.95,0.342996571428571)
		(6.96,0.342511047619048)
		(6.97,0.342996571428571)
		(6.98,0.343482095238095)
		(6.99,0.343239333333333)
		(7,0.343117952380952)
		(7.01,0.343239333333333)
		(7.02,0.343360714285714)
		(7.03,0.342996571428571)
		(7.04,0.34287519047619)
		(7.05,0.343117952380952)
		(7.06,0.34287519047619)
		(7.07,0.34287519047619)
		(7.08,0.342389666666667)
		(7.09,0.342025523809524)
		(7.1,0.342146904761905)
		(7.11,0.342268285714286)
		(7.12,0.34154)
		(7.13,0.341175857142857)
		(7.14,0.341175857142857)
		(7.15,0.341175857142857)
		(7.16,0.341297238095238)
		(7.17,0.34154)
		(7.18,0.341054476190476)
		(7.19,0.340568952380952)
		(7.2,0.340690333333333)
		(7.21,0.340568952380952)
		(7.22,0.340204809523809)
		(7.23,0.340083428571428)
		(7.24,0.340204809523809)
		(7.25,0.340204809523809)
		(7.26,0.34032619047619)
		(7.27,0.340204809523809)
		(7.28,0.34032619047619)
		(7.29,0.340204809523809)
		(7.3,0.34032619047619)
		(7.31,0.34032619047619)
		(7.32,0.340568952380952)
		(7.33,0.340811714285714)
		(7.34,0.340690333333333)
		(7.35,0.340447571428571)
		(7.36,0.340447571428571)
		(7.37,0.339840666666667)
		(7.38,0.339112380952381)
		(7.39,0.338991)
		(7.4,0.339233761904762)
		(7.41,0.339355142857143)
		(7.42,0.338869619047619)
		(7.43,0.338869619047619)
		(7.44,0.338869619047619)
		(7.45,0.338262714285714)
		(7.46,0.338141333333333)
		(7.47,0.337655809523809)
		(7.48,0.337534428571429)
		(7.49,0.337534428571429)
		(7.5,0.337898571428571)
		(7.51,0.337655809523809)
		(7.52,0.337534428571429)
		(7.53,0.337534428571428)
		(7.54,0.337413047619048)
		(7.55,0.337048904761905)
		(7.56,0.337170285714286)
		(7.57,0.336927523809524)
		(7.58,0.337048904761905)
		(7.59,0.337655809523809)
		(7.6,0.337898571428571)
		(7.61,0.337534428571428)
		(7.62,0.336806142857143)
		(7.63,0.337413047619048)
		(7.64,0.337048904761905)
		(7.65,0.337048904761905)
		(7.66,0.337534428571429)
		(7.67,0.337170285714286)
		(7.68,0.336806142857143)
		(7.69,0.336806142857143)
		(7.7,0.337048904761905)
		(7.71,0.337170285714286)
		(7.72,0.337048904761905)
		(7.73,0.337048904761905)
		(7.74,0.336442)
		(7.75,0.336442)
		(7.76,0.336927523809524)
		(7.77,0.336684761904762)
		(7.78,0.336684761904762)
		(7.79,0.336684761904762)
		(7.8,0.336320619047619)
		(7.81,0.336077857142857)
		(7.82,0.336320619047619)
		(7.83,0.336927523809524)
		(7.84,0.336563380952381)
		(7.85,0.336806142857143)
		(7.86,0.337048904761905)
		(7.87,0.337048904761905)
		(7.88,0.337655809523809)
		(7.89,0.338019952380952)
		(7.9,0.337655809523809)
		(7.91,0.337291666666667)
		(7.92,0.337048904761905)
		(7.93,0.337048904761905)
		(7.94,0.337170285714286)
		(7.95,0.337048904761905)
		(7.96,0.336684761904762)
		(7.97,0.336684761904762)
		(7.98,0.336684761904762)
		(7.99,0.336806142857143)
		(8,0.336442)
		(8.01,0.336320619047619)
		(8.02,0.336684761904762)
		(8.03,0.336684761904762)
		(8.04,0.336684761904762)
		(8.05,0.336442)
		(8.06,0.336077857142857)
		(8.07,0.336077857142857)
		(8.08,0.335835095238095)
		(8.09,0.335592333333333)
		(8.1,0.335713714285714)
		(8.11,0.336077857142857)
		(8.12,0.336077857142857)
		(8.13,0.335713714285714)
		(8.14,0.335592333333333)
		(8.15,0.335713714285714)
		(8.16,0.335956476190476)
		(8.17,0.336199238095238)
		(8.18,0.336077857142857)
		(8.19,0.336320619047619)
		(8.2,0.336320619047619)
		(8.21,0.336806142857143)
		(8.22,0.336684761904762)
		(8.23,0.336442)
		(8.24,0.336077857142857)
		(8.25,0.336077857142857)
		(8.26,0.336563380952381)
		(8.27,0.336806142857143)
		(8.28,0.336442)
		(8.29,0.336320619047619)
		(8.3,0.336199238095238)
		(8.31,0.335835095238095)
		(8.32,0.335592333333333)
		(8.33,0.335349571428571)
		(8.34,0.335470952380952)
		(8.35,0.335470952380952)
		(8.36,0.334864047619048)
		(8.37,0.334621285714286)
		(8.38,0.334378523809524)
		(8.39,0.333771619047619)
		(8.4,0.333043333333333)
		(8.41,0.332921952380952)
		(8.42,0.332921952380952)
		(8.43,0.332800571428571)
		(8.44,0.332921952380952)
		(8.45,0.332921952380952)
		(8.46,0.332557809523809)
		(8.47,0.33267919047619)
		(8.48,0.332557809523809)
		(8.49,0.332557809523809)
		(8.5,0.332557809523809)
		(8.51,0.332800571428571)
		(8.52,0.332557809523809)
		(8.53,0.332921952380952)
		(8.54,0.332800571428571)
		(8.55,0.332921952380952)
		(8.56,0.332921952380952)
		(8.57,0.333164714285714)
		(8.58,0.333407476190476)
		(8.59,0.333893)
		(8.6,0.333893)
		(8.61,0.334257142857143)
		(8.62,0.334014380952381)
		(8.63,0.334014380952381)
		(8.64,0.334257142857143)
		(8.65,0.334135761904762)
		(8.66,0.333771619047619)
		(8.67,0.333771619047619)
		(8.68,0.333286095238095)
		(8.69,0.333286095238095)
		(8.7,0.333164714285714)
		(8.71,0.333164714285714)
		(8.72,0.332800571428571)
		(8.73,0.333407476190476)
		(8.74,0.333164714285714)
		(8.75,0.333407476190476)
		(8.76,0.333286095238095)
		(8.77,0.333164714285714)
		(8.78,0.333407476190476)
		(8.79,0.333043333333333)
		(8.8,0.33267919047619)
		(8.81,0.333286095238095)
		(8.82,0.332921952380952)
		(8.83,0.332921952380952)
		(8.84,0.332921952380952)
		(8.85,0.333164714285714)
		(8.86,0.333043333333333)
		(8.87,0.333164714285714)
		(8.88,0.333164714285714)
		(8.89,0.333528857142857)
		(8.9,0.333286095238095)
		(8.91,0.333407476190476)
		(8.92,0.333407476190476)
		(8.93,0.333407476190476)
		(8.94,0.333043333333333)
		(8.95,0.332800571428571)
		(8.96,0.332921952380952)
		(8.97,0.333286095238095)
		(8.98,0.333164714285714)
		(8.99,0.333164714285714)
		};

==> addplot__TransmTest_DetectedEdges.tex <==
\addplot [red] coordinates{
	(0,0)
(0.01,0)
(0.02,0)
(0.03,0)
(0.04,0)
(0.05,0)
(0.06,0)
(0.07,0)
(0.08,0)
(0.09,0)
(0.1,0)
(0.11,0)
(0.12,0)
(0.13,0)
(0.14,0)
(0.15,0)
(0.16,0)
(0.17,0)
(0.18,0)
(0.19,0)
(0.2,0)
(0.21,0)
(0.22,0)
(0.23,0)
(0.24,0)
(0.25,0)
(0.26,0)
(0.27,0)
(0.28,0)
(0.29,0)
(0.3,0)
(0.31,0)
(0.32,0)
(0.33,0)
(0.34,0)
(0.35,0)
(0.36,0)
(0.37,0)
(0.38,0)
(0.39,0)
(0.4,0)
(0.41,0)
(0.42,0)
(0.43,0)
(0.44,0)
(0.45,0)
(0.46,0)
(0.47,0)
(0.48,0)
(0.49,0)
(0.5,0)
(0.51,0)
(0.52,0)
(0.53,0)
(0.54,0)
(0.55,0)
(0.56,0)
(0.57,0)
(0.58,0)
(0.59,0)
(0.6,0)
(0.61,0)
(0.62,0)
(0.63,0)
(0.64,0)
(0.65,0)
(0.66,0)
(0.67,0)
(0.68,0)
(0.69,0)
(0.7,0)
(0.71,0)
(0.72,0)
(0.73,0)
(0.74,0)
(0.75,0)
(0.76,0)
(0.77,0)
(0.78,0)
(0.79,0)
(0.8,0)
(0.81,0)
(0.82,0)
(0.83,0)
(0.84,0)
(0.85,0)
(0.86,0)
(0.87,0)
(0.88,0)
(0.89,0)
(0.9,0)
(0.91,0)
(0.92,0)
(0.93,0)
(0.94,0)
(0.95,0)
(0.96,0)
(0.97,0)
(0.98,0)
(0.99,0)
(1,0)
(1.01,0)
(1.02,0)
(1.03,0)
(1.04,0)
(1.05,0)
(1.06,0)
(1.07,0)
(1.08,0)
(1.09,0)
(1.1,0)
(1.11,0)
(1.12,0)
(1.13,0)
(1.14,0)
(1.15,0)
(1.16,0)
(1.17,0)
(1.18,0)
(1.19,0)
(1.2,0)
(1.21,0)
(1.22,0)
(1.23,0)
(1.24,0)
(1.25,0)
(1.26,0)
(1.27,0)
(1.28,0)
(1.29,0)
(1.3,0)
(1.31,0)
(1.32,0)
(1.33,0)
(1.34,0)
(1.35,0)
(1.36,0)
(1.37,0)
(1.38,0)
(1.39,0)
(1.4,0)
(1.41,0)
(1.42,0)
(1.43,0)
(1.44,0)
(1.45,0)
(1.46,0)
(1.47,0)
(1.48,0)
(1.49,0)
(1.5,0)
(1.51,0)
(1.52,0)
(1.53,0)
(1.54,0)
(1.55,0)
(1.56,0)
(1.57,0)
(1.58,0)
(1.59,0)
(1.6,0)
(1.61,0)
(1.62,0)
(1.63,0)
(1.64,0)
(1.65,0)
(1.66,0)
(1.67,0)
(1.68,0)
(1.69,0)
(1.7,0)
(1.71,0)
(1.72,0)
(1.73,0)
(1.74,0)
(1.75,0)
(1.76,0)
(1.77,0)
(1.78,0)
(1.79,0)
(1.8,0)
(1.81,0)
(1.82,0)
(1.83,0)
(1.84,0)
(1.85,0)
(1.86,0)
(1.87,0)
(1.88,0)
(1.89,0)
(1.9,0)
(1.91,0)
(1.92,0)
(1.93,0)
(1.94,0)
(1.95,0)
(1.96,0)
(1.97,0)
(1.98,0)
(1.99,0)
(2,1)
(2.01,1)
(2.02,1)
(2.03,1)
(2.04,1)
(2.05,1)
(2.06,1)
(2.07,1)
(2.08,1)
(2.09,1)
(2.1,1)
(2.11,1)
(2.12,1)
(2.13,1)
(2.14,1)
(2.15,1)
(2.16,1)
(2.17,1)
(2.18,1)
(2.19,1)
(2.2,1)
(2.21,1)
(2.22,1)
(2.23,1)
(2.24,1)
(2.25,1)
(2.26,1)
(2.27,1)
(2.28,1)
(2.29,1)
(2.3,1)
(2.31,1)
(2.32,1)
(2.33,1)
(2.34,1)
(2.35,1)
(2.36,1)
(2.37,1)
(2.38,1)
(2.39,1)
(2.4,1)
(2.41,1)
(2.42,1)
(2.43,1)
(2.44,1)
(2.45,1)
(2.46,1)
(2.47,0)
(2.48,0)
(2.49,0)
(2.5,0)
(2.51,0)
(2.52,0)
(2.53,0)
(2.54,0)
(2.55,0)
(2.56,0)
(2.57,0)
(2.58,0)
(2.59,0)
(2.6,0)
(2.61,0)
(2.62,0)
(2.63,0)
(2.64,0)
(2.65,0)
(2.66,0)
(2.67,0)
(2.68,0)
(2.69,0)
(2.7,0)
(2.71,0)
(2.72,0)
(2.73,0)
(2.74,0)
(2.75,0)
(2.76,0)
(2.77,0)
(2.78,0)
(2.79,0)
(2.8,0)
(2.81,0)
(2.82,0)
(2.83,0)
(2.84,0)
(2.85,0)
(2.86,0)
(2.87,0)
(2.88,0)
(2.89,0)
(2.9,0)
(2.91,0)
(2.92,0)
(2.93,0)
(2.94,0)
(2.95,0)
(2.96,0)
(2.97,0)
(2.98,0)
(2.99,0)
(3,0)
(3.01,0)
(3.02,0)
(3.03,0)
(3.04,0)
(3.05,0)
(3.06,0)
(3.07,0)
(3.08,0)
(3.09,0)
(3.1,0)
(3.11,0)
(3.12,0)
(3.13,0)
(3.14,0)
(3.15,0)
(3.16,0)
(3.17,0)
(3.18,0)
(3.19,0)
(3.2,0)
(3.21,0)
(3.22,0)
(3.23,0)
(3.24,0)
(3.25,0)
(3.26,0)
(3.27,0)
(3.28,0)
(3.29,0)
(3.3,0)
(3.31,0)
(3.32,0)
(3.33,0)
(3.34,0)
(3.35,0)
(3.36,0)
(3.37,0)
(3.38,0)
(3.39,0)
(3.4,0)
(3.41,0)
(3.42,0)
(3.43,0)
(3.44,0)
(3.45,0)
(3.46,0)
(3.47,0)
(3.48,0)
(3.49,0)
(3.5,0)
(3.51,0)
(3.52,0)
(3.53,0)
(3.54,0)
(3.55,0)
(3.56,0)
(3.57,0)
(3.58,0)
(3.59,0)
(3.6,0)
(3.61,0)
(3.62,0)
(3.63,0)
(3.64,0)
(3.65,0)
(3.66,0)
(3.67,0)
(3.68,0)
(3.69,0)
(3.7,0)
(3.71,0)
(3.72,0)
(3.73,0)
(3.74,0)
(3.75,0)
(3.76,0)
(3.77,0)
(3.78,0)
(3.79,0)
(3.8,0)
(3.81,0)
(3.82,0)
(3.83,0)
(3.84,0)
(3.85,0)
(3.86,0)
(3.87,0)
(3.88,0)
(3.89,0)
(3.9,0)
(3.91,0)
(3.92,0)
(3.93,0)
(3.94,0)
(3.95,0)
(3.96,0)
(3.97,0)
(3.98,0)
(3.99,0)
(4,0)
(4.01,0)
(4.02,0)
(4.03,0)
(4.04,0)
(4.05,0)
(4.06,0)
(4.07,0)
(4.08,0)
(4.09,0)
(4.1,0)
(4.11,0)
(4.12,0)
(4.13,0)
(4.14,0)
(4.15,0)
(4.16,0)
(4.17,0)
(4.18,0)
(4.19,0)
(4.2,0)
(4.21,0)
(4.22,0)
(4.23,0)
(4.24,0)
(4.25,0)
(4.26,0)
(4.27,0)
(4.28,0)
(4.29,0)
(4.3,0)
(4.31,0)
(4.32,0)
(4.33,0)
(4.34,0)
(4.35,0)
(4.36,0)
(4.37,0)
(4.38,0)
(4.39,0)
(4.4,0)
(4.41,0)
(4.42,0)
(4.43,0)
(4.44,0)
(4.45,0)
(4.46,0)
(4.47,0)
(4.48,0)
(4.49,0)
(4.5,0)
(4.51,0)
(4.52,0)
(4.53,0)
(4.54,0)
(4.55,0)
(4.56,0)
(4.57,0)
(4.58,0)
(4.59,0)
(4.6,0)
(4.61,0)
(4.62,0)
(4.63,0)
(4.64,0)
(4.65,0)
(4.66,0)
(4.67,0)
(4.68,0)
(4.69,0)
(4.7,0)
(4.71,0)
(4.72,0)
(4.73,0)
(4.74,0)
(4.75,0)
(4.76,0)
(4.77,0)
(4.78,0)
(4.79,0)
(4.8,0)
(4.81,0)
(4.82,0)
(4.83,0)
(4.84,1)
(4.85,1)
(4.86,1)
(4.87,1)
(4.88,1)
(4.89,1)
(4.9,1)
(4.91,1)
(4.92,1)
(4.93,1)
(4.94,1)
(4.95,1)
(4.96,1)
(4.97,1)
(4.98,1)
(4.99,1)
(5,1)
(5.01,1)
(5.02,1)
(5.03,1)
(5.04,1)
(5.05,1)
(5.06,1)
(5.07,1)
(5.08,1)
(5.09,1)
(5.1,1)
(5.11,1)
(5.12,1)
(5.13,1)
(5.14,1)
(5.15,1)
(5.16,1)
(5.17,1)
(5.18,1)
(5.19,1)
(5.2,1)
(5.21,1)
(5.22,1)
(5.23,1)
(5.24,1)
(5.25,1)
(5.26,1)
(5.27,1)
(5.28,1)
(5.29,1)
(5.3,1)
(5.31,1)
(5.32,1)
(5.33,1)
(5.34,1)
(5.35,1)
(5.36,1)
(5.37,1)
(5.38,1)
(5.39,1)
(5.4,1)
(5.41,1)
(5.42,1)
(5.43,1)
(5.44,1)
(5.45,1)
(5.46,1)
(5.47,1)
(5.48,1)
(5.49,1)
(5.5,0)
(5.51,0)
(5.52,0)
(5.53,0)
(5.54,0)
(5.55,0)
(5.56,0)
(5.57,0)
(5.58,0)
(5.59,0)
(5.6,0)
(5.61,0)
(5.62,0)
(5.63,0)
(5.64,0)
(5.65,0)
(5.66,0)
(5.67,0)
(5.68,0)
(5.69,0)
(5.7,0)
(5.71,0)
(5.72,0)
(5.73,0)
(5.74,0)
(5.75,0)
(5.76,0)
(5.77,0)
(5.78,0)
(5.79,0)
(5.8,0)
(5.81,0)
(5.82,0)
(5.83,0)
(5.84,0)
(5.85,0)
(5.86,0)
(5.87,0)
(5.88,0)
(5.89,0)
(5.9,0)
(5.91,0)
(5.92,0)
(5.93,0)
(5.94,0)
(5.95,0)
(5.96,0)
(5.97,0)
(5.98,0)
(5.99,0)
(6,0)
(6.01,0)
(6.02,0)
(6.03,0)
(6.04,0)
(6.05,0)
(6.06,0)
(6.07,0)
(6.08,0)
(6.09,0)
(6.1,0)
(6.11,0)
(6.12,0)
(6.13,0)
(6.14,0)
(6.15,0)
(6.16,0)
(6.17,0)
(6.18,0)
(6.19,0)
(6.2,0)
(6.21,0)
(6.22,0)
(6.23,0)
(6.24,0)
(6.25,0)
(6.26,0)
(6.27,0)
(6.28,0)
(6.29,0)
(6.3,0)
(6.31,0)
(6.32,0)
(6.33,0)
(6.34,0)
(6.35,0)
(6.36,0)
(6.37,0)
(6.38,0)
(6.39,0)
(6.4,0)
(6.41,0)
(6.42,0)
(6.43,0)
(6.44,0)
(6.45,0)
(6.46,0)
(6.47,0)
(6.48,0)
(6.49,0)
(6.5,0)
(6.51,0)
(6.52,0)
(6.53,0)
(6.54,0)
(6.55,0)
(6.56,0)
(6.57,0)
(6.58,0)
(6.59,0)
(6.6,0)
(6.61,0)
(6.62,0)
(6.63,0)
(6.64,0)
(6.65,0)
(6.66,0)
(6.67,0)
(6.68,0)
(6.69,0)
(6.7,0)
(6.71,0)
(6.72,0)
(6.73,0)
(6.74,0)
(6.75,0)
(6.76,0)
(6.77,0)
(6.78,0)
(6.79,0)
(6.8,1)
(6.81,1)
(6.82,1)
(6.83,1)
(6.84,1)
(6.85,1)
(6.86,1)
(6.87,1)
(6.88,1)
(6.89,1)
(6.9,1)
(6.91,1)
(6.92,1)
(6.93,1)
(6.94,1)
(6.95,1)
(6.96,1)
(6.97,1)
(6.98,1)
(6.99,1)
(7,1)
(7.01,1)
(7.02,1)
(7.03,1)
(7.04,1)
(7.05,1)
(7.06,1)
(7.07,1)
(7.08,1)
(7.09,1)
(7.1,1)
(7.11,1)
(7.12,1)
(7.13,1)
(7.14,1)
(7.15,1)
(7.16,1)
(7.17,1)
(7.18,1)
(7.19,1)
(7.2,1)
(7.21,1)
(7.22,1)
(7.23,1)
(7.24,1)
(7.25,1)
(7.26,1)
(7.27,1)
(7.28,1)
(7.29,1)
(7.3,1)
(7.31,1)
(7.32,1)
(7.33,1)
(7.34,1)
(7.35,1)
(7.36,1)
(7.37,1)
(7.38,1)
(7.39,1)
(7.4,1)
(7.41,1)
(7.42,1)
(7.43,1)
(7.44,1)
(7.45,1)
(7.46,1)
(7.47,1)
(7.48,1)
(7.49,1)
(7.5,1)
(7.51,1)
(7.52,0)
(7.53,0)
(7.54,0)
(7.55,0)
(7.56,0)
(7.57,0)
(7.58,0)
(7.59,0)
(7.6,0)
(7.61,0)
(7.62,0)
(7.63,0)
(7.64,0)
(7.65,0)
(7.66,0)
(7.67,0)
(7.68,0)
(7.69,0)
(7.7,0)
(7.71,1)
(7.72,1)
(7.73,1)
(7.74,1)
(7.75,1)
(7.76,1)
(7.77,1)
(7.78,1)
(7.79,1)
(7.8,1)
(7.81,1)
(7.82,1)
(7.83,1)
(7.84,1)
(7.85,1)
(7.86,1)
(7.87,1)
(7.88,1)
(7.89,1)
(7.9,1)
(7.91,1)
(7.92,1)
(7.93,1)
(7.94,1)
(7.95,1)
(7.96,1)
(7.97,1)
(7.98,1)
(7.99,1)
(8,1)
(8.01,1)
(8.02,1)
(8.03,1)
(8.04,1)
(8.05,1)
(8.06,1)
(8.07,1)
(8.08,1)
(8.09,1)
(8.1,1)
(8.11,1)
(8.12,1)
(8.13,1)
(8.14,1)
(8.15,1)
(8.16,1)
(8.17,1)
(8.18,1)
(8.19,1)
(8.2,1)
(8.21,1)
(8.22,1)
(8.23,1)
(8.24,1)
(8.25,1)
(8.26,1)
(8.27,1)
(8.28,1)
(8.29,1)
(8.3,1)
(8.31,1)
(8.32,1)
(8.33,1)
(8.34,1)
(8.35,1)
(8.36,1)
(8.37,1)
(8.38,1)
(8.39,1)
(8.4,1)
(8.41,1)
(8.42,1)
(8.43,1)
(8.44,1)
(8.45,1)
(8.46,1)
(8.47,1)
(8.48,1)
(8.49,1)
(8.5,1)
(8.51,1)
(8.52,1)
(8.53,1)
(8.54,1)
(8.55,1)
(8.56,1)
(8.57,1)
(8.58,0)
(8.59,0)
(8.6,0)
(8.61,0)
(8.62,0)
(8.63,0)
(8.64,0)
(8.65,0)
(8.66,0)
(8.67,0)
(8.68,0)
(8.69,0)
(8.7,0)
(8.71,0)
(8.72,0)
(8.73,0)
(8.74,0)
(8.75,0)
(8.76,0)
(8.77,0)
(8.78,0)
(8.79,0)
(8.8,0)
(8.81,0)
(8.82,0)
(8.83,0)
(8.84,0)
(8.85,0)
(8.86,0)
(8.87,0)
(8.88,0)
(8.89,0)
(8.9,0)
(8.91,0)
(8.92,0)
(8.93,0)
(8.94,0)
(8.95,0)
(8.96,0)
(8.97,0)
(8.98,0)
(8.99,0)
(9,0)
(9.01,0)
(9.02,0)
(9.03,0)
(9.04,0)
(9.05,0)
(9.06,0)
(9.07,0)
(9.08,0)
(9.09,0)
(9.1,0)
(9.11,0)
(9.12,0)
(9.13,0)
(9.14,0)
(9.15,0)
(9.16,0)
(9.17,0)
(9.18,0)
(9.19,0)
(9.2,0)
(9.21,0)
(9.22,0)
(9.23,0)
(9.24,0)
(9.25,0)
(9.26,0)
(9.27,0)
(9.28,0)
(9.29,0)
(9.3,0)
(9.31,0)
(9.32,0)
(9.33,0)
(9.34,0)
(9.35,0)
(9.36,0)
(9.37,0)
(9.38,0)
(9.39,0)
(9.4,0)
(9.41,0)
(9.42,0)
(9.43,0)
(9.44,0)
(9.45,0)
(9.46,0)
(9.47,0)
(9.48,0)
(9.49,0)
(9.5,0)
(9.51,0)
(9.52,0)
(9.53,0)
(9.54,0)
(9.55,0)
(9.56,0)
(9.57,0)
(9.58,0)
(9.59,0)
(9.6,0)
(9.61,0)
(9.62,0)
(9.63,0)
(9.64,0)
(9.65,0)
(9.66,0)
(9.67,0)
(9.68,0)
(9.69,0)
(9.7,0)
(9.71,0)
(9.72,0)
(9.73,0)
(9.74,0)
(9.75,0)
(9.76,0)
(9.77,0)
(9.78,0)
(9.79,0)
(9.8,0)
(9.81,0)
(9.82,0)
(9.83,0)
(9.84,0)
(9.85,0)
(9.86,0)
(9.87,0)
(9.88,0)
(9.89,0)
(9.9,0)
(9.91,0)
(9.92,0)
(9.93,0)
(9.94,0)
(9.95,0)
(9.96,0)
(9.97,0)
(9.98,0)
(9.99,0)
(10,0)
(10.01,0)
(10.02,0)
(10.03,0)
(10.04,0)
(10.05,0)
(10.06,0)
(10.07,0)
(10.08,0)
(10.09,0)
(10.1,0)
(10.11,0)
(10.12,0)
(10.13,0)
(10.14,0)
(10.15,0)
(10.16,0)
(10.17,0)
(10.18,0)
(10.19,0)
(10.2,0)
(10.21,0)
(10.22,0)
(10.23,0)
(10.24,0)
(10.25,0)
(10.26,0)
(10.27,0)
(10.28,0)
(10.29,0)
(10.3,0)
(10.31,0)
(10.32,0)
(10.33,0)
(10.34,0)
(10.35,0)
(10.36,0)
(10.37,0)
(10.38,0)
(10.39,0)
(10.4,0)
(10.41,0)
(10.42,0)
(10.43,0)
(10.44,0)
(10.45,0)
(10.46,0)
(10.47,0)
(10.48,0)
(10.49,0)
(10.5,0)
(10.51,0)
(10.52,0)
(10.53,0)
(10.54,0)
(10.55,0)
(10.56,0)
(10.57,0)
(10.58,0)
(10.59,0)
(10.6,0)
(10.61,0)
(10.62,0)
(10.63,0)
(10.64,0)
(10.65,0)
(10.66,0)
(10.67,0)
(10.68,0)
(10.69,0)
(10.7,0)
(10.71,0)
(10.72,0)
(10.73,0)
(10.74,0)
(10.75,0)
(10.76,0)
(10.77,0)
(10.78,0)
(10.79,0)
(10.8,0)
(10.81,0)
(10.82,0)
(10.83,0)
(10.84,0)
(10.85,0)
(10.86,0)
(10.87,0)
(10.88,0)
(10.89,0)
(10.9,0)
(10.91,0)
(10.92,0)
(10.93,0)
(10.94,0)
(10.95,0)
(10.96,0)
(10.97,0)
(10.98,0)
(10.99,0)
(11,0)
(11.01,0)
(11.02,0)
(11.03,0)
(11.04,0)
(11.05,0)
(11.06,0)
(11.07,0)
(11.08,0)
(11.09,0)
(11.1,0)
(11.11,0)
(11.12,0)
(11.13,0)
(11.14,0)
(11.15,0)
(11.16,0)
(11.17,0)
(11.18,0)
(11.19,0)
(11.2,0)
(11.21,0)
(11.22,0)
(11.23,0)
(11.24,0)
(11.25,0)
(11.26,0)
(11.27,0)
(11.28,0)
(11.29,0)
(11.3,0)
(11.31,0)
(11.32,0)
(11.33,0)
(11.34,0)
(11.35,0)
(11.36,0)
(11.37,0)
(11.38,0)
(11.39,0)
(11.4,0)
(11.41,0)
(11.42,0)
(11.43,0)
(11.44,0)
(11.45,0)
(11.46,0)
(11.47,0)
(11.48,0)
(11.49,0)
(11.5,0)
(11.51,0)
(11.52,0)
(11.53,0)
(11.54,0)
(11.55,0)
(11.56,0)
(11.57,0)
(11.58,0)
(11.59,0)
(11.6,0)
(11.61,0)
(11.62,0)
(11.63,0)
(11.64,0)
(11.65,0)
(11.66,0)
(11.67,0)
(11.68,0)
(11.69,0)
(11.7,0)
(11.71,0)
(11.72,0)
(11.73,0)
(11.74,0)
(11.75,0)
(11.76,0)
(11.77,0)
(11.78,0)
(11.79,0)
(11.8,0)
(11.81,0)
(11.82,0)
(11.83,0)
(11.84,0)
(11.85,0)
(11.86,0)
(11.87,0)
(11.88,0)
(11.89,0)
(11.9,0)
(11.91,0)
(11.92,0)
(11.93,0)
(11.94,0)
(11.95,0)
(11.96,0)
(11.97,0)
(11.98,0)
(11.99,0)
(12,0)
(12.01,0)
(12.02,0)
(12.03,0)
(12.04,0)
(12.05,0)
(12.06,0)
(12.07,0)
(12.08,0)
(12.09,0)
(12.1,0)
(12.11,0)
(12.12,0)
(12.13,0)
(12.14,0)
(12.15,0)
(12.16,0)
(12.17,0)
(12.18,0)
(12.19,0)
(12.2,0)
(12.21,0)
(12.22,0)
(12.23,0)
(12.24,0)
(12.25,0)
(12.26,0)
(12.27,0)
(12.28,0)
(12.29,0)
(12.3,0)
(12.31,0)
(12.32,0)
(12.33,0)
(12.34,0)
(12.35,0)
(12.36,0)
(12.37,0)
(12.38,0)
(12.39,0)
(12.4,0)
(12.41,0)
(12.42,0)
(12.43,0)
(12.44,0)
(12.45,0)
(12.46,0)
(12.47,0)
(12.48,0)
(12.49,0)
(12.5,0)
(12.51,0)
(12.52,0)
(12.53,0)
(12.54,0)
(12.55,0)
(12.56,0)
(12.57,0)
(12.58,0)
(12.59,0)
(12.6,0)
(12.61,0)
(12.62,0)
(12.63,0)
(12.64,0)
(12.65,0)
(12.66,0)
(12.67,0)
(12.68,0)
(12.69,0)
(12.7,0)
(12.71,0)
(12.72,0)
(12.73,0)
(12.74,0)
(12.75,0)
(12.76,0)
(12.77,0)
(12.78,0)
(12.79,0)
(12.8,0)
(12.81,0)
(12.82,0)
(12.83,0)
(12.84,0)
(12.85,0)
(12.86,0)
(12.87,0)
(12.88,0)
(12.89,0)
(12.9,0)
(12.91,0)
(12.92,0)
(12.93,0)
(12.94,0)
(12.95,0)
(12.96,0)
(12.97,0)
(12.98,0)
(12.99,0)
(13,0)
(13.01,0)
(13.02,0)
(13.03,0)
(13.04,0)
(13.05,0)
(13.06,0)
(13.07,0)
(13.08,0)
(13.09,0)
(13.1,0)
(13.11,0)
(13.12,0)
(13.13,0)
(13.14,0)
(13.15,0)
(13.16,0)
(13.17,0)
(13.18,0)
(13.19,0)
(13.2,0)
(13.21,0)
(13.22,0)
(13.23,0)
(13.24,0)
(13.25,0)
(13.26,0)
(13.27,0)
(13.28,0)
(13.29,0)
(13.3,0)
(13.31,0)
(13.32,0)
(13.33,0)
(13.34,0)
(13.35,0)
(13.36,0)
(13.37,0)
(13.38,0)
(13.39,0)
(13.4,0)
(13.41,0)
(13.42,0)
(13.43,0)
(13.44,0)
(13.45,0)
(13.46,0)
(13.47,0)
(13.48,0)
(13.49,0)
(13.5,0)
(13.51,0)
(13.52,0)
(13.53,0)
(13.54,0)
(13.55,0)
(13.56,0)
(13.57,0)
(13.58,0)
(13.59,0)
(13.6,0)
(13.61,0)
(13.62,0)
(13.63,0)
(13.64,0)
(13.65,0)
(13.66,0)
(13.67,0)
(13.68,0)
(13.69,0)
(13.7,0)
(13.71,0)
(13.72,0)
(13.73,0)
(13.74,0)
(13.75,0)
(13.76,0)
(13.77,0)
(13.78,0)
(13.79,0)
(13.8,0)
(13.81,0)
(13.82,0)
(13.83,0)
(13.84,1)
(13.85,1)
(13.86,1)
(13.87,1)
(13.88,1)
(13.89,1)
(13.9,1)
(13.91,1)
(13.92,1)
(13.93,1)
(13.94,1)
(13.95,1)
(13.96,1)
(13.97,1)
(13.98,1)
(13.99,1)
(14,1)
(14.01,1)
(14.02,1)
(14.03,1)
(14.04,1)
(14.05,1)
(14.06,1)
(14.07,1)
(14.08,1)
(14.09,1)
(14.1,1)
(14.11,1)
(14.12,1)
(14.13,1)
(14.14,1)
(14.15,1)
(14.16,1)
(14.17,1)
(14.18,1)
(14.19,1)
(14.2,1)
(14.21,1)
(14.22,1)
(14.23,1)
(14.24,1)
(14.25,1)
(14.26,1)
(14.27,1)
(14.28,1)
(14.29,1)
(14.3,1)
(14.31,1)
(14.32,1)
(14.33,1)
(14.34,1)
(14.35,1)
(14.36,1)
(14.37,1)
(14.38,1)
(14.39,1)
(14.4,1)
(14.41,1)
(14.42,1)
(14.43,1)
(14.44,1)
(14.45,1)
(14.46,1)
(14.47,1)
(14.48,1)
(14.49,1)
(14.5,0)
(14.51,0)
(14.52,0)
(14.53,0)
(14.54,0)
(14.55,0)
(14.56,0)
(14.57,0)
(14.58,0)
(14.59,0)
(14.6,0)
(14.61,0)
(14.62,0)
(14.63,0)
(14.64,0)
(14.65,0)
(14.66,0)
(14.67,0)
(14.68,0)
(14.69,0)
(14.7,1)
(14.71,1)
(14.72,1)
(14.73,1)
(14.74,1)
(14.75,1)
(14.76,1)
(14.77,1)
(14.78,1)
(14.79,1)
(14.8,1)
(14.81,1)
(14.82,1)
(14.83,1)
(14.84,1)
(14.85,1)
(14.86,1)
(14.87,1)
(14.88,1)
(14.89,1)
(14.9,1)
(14.91,1)
(14.92,1)
(14.93,1)
(14.94,1)
(14.95,1)
(14.96,1)
(14.97,1)
(14.98,1)
(14.99,1)
(15,1)
(15.01,1)
(15.02,1)
(15.03,1)
(15.04,1)
(15.05,1)
(15.06,1)
(15.07,1)
(15.08,1)
(15.09,1)
(15.1,1)
(15.11,1)
(15.12,1)
(15.13,1)
(15.14,1)
(15.15,1)
(15.16,1)
(15.17,1)
(15.18,1)
(15.19,1)
(15.2,1)
(15.21,1)
(15.22,1)
(15.23,1)
(15.24,1)
(15.25,1)
(15.26,1)
(15.27,1)
(15.28,1)
(15.29,1)
(15.3,1)
(15.31,1)
(15.32,1)
(15.33,1)
(15.34,1)
(15.35,1)
(15.36,1)
(15.37,1)
(15.38,1)
(15.39,1)
(15.4,1)
(15.41,1)
(15.42,1)
(15.43,1)
(15.44,1)
(15.45,1)
(15.46,1)
(15.47,1)
(15.48,1)
(15.49,1)
(15.5,1)
(15.51,1)
(15.52,1)
(15.53,1)
(15.54,1)
(15.55,0)
(15.56,0)
(15.57,0)
(15.58,0)
(15.59,0)
(15.6,0)
(15.61,0)
(15.62,0)
(15.63,0)
(15.64,0)
(15.65,0)
(15.66,0)
(15.67,0)
(15.68,0)
(15.69,0)
(15.7,0)
(15.71,0)
(15.72,0)
(15.73,0)
(15.74,0)
(15.75,0)
(15.76,0)
(15.77,0)
(15.78,0)
(15.79,0)
(15.8,0)
(15.81,0)
(15.82,0)
(15.83,0)
(15.84,0)
(15.85,0)
(15.86,0)
(15.87,0)
(15.88,0)
(15.89,0)
(15.9,0)
(15.91,0)
(15.92,0)
(15.93,0)
(15.94,0)
(15.95,0)
(15.96,0)
(15.97,0)
(15.98,0)
(15.99,0)
(16,0)
(16.01,0)
(16.02,0)
(16.03,0)
(16.04,0)
(16.05,0)
(16.06,0)
(16.07,0)
(16.08,0)
(16.09,0)
(16.1,0)
(16.11,0)
(16.12,0)
(16.13,0)
(16.14,0)
(16.15,0)
(16.16,0)
(16.17,0)
(16.18,0)
(16.19,0)
(16.2,0)
(16.21,0)
(16.22,0)
(16.23,0)
(16.24,0)
(16.25,0)
(16.26,0)
(16.27,0)
(16.28,0)
(16.29,0)
(16.3,0)
(16.31,0)
(16.32,0)
(16.33,0)
(16.34,0)
(16.35,0)
(16.36,0)
(16.37,0)
(16.38,0)
(16.39,0)
(16.4,0)
(16.41,0)
(16.42,0)
(16.43,0)
(16.44,0)
(16.45,0)
(16.46,0)
(16.47,0)
(16.48,0)
(16.49,0)
(16.5,0)
(16.51,0)
(16.52,0)
(16.53,0)
(16.54,0)
(16.55,0)
(16.56,0)
(16.57,0)
(16.58,0)
(16.59,0)
(16.6,0)
(16.61,0)
(16.62,0)
(16.63,0)
(16.64,0)
(16.65,0)
(16.66,0)
(16.67,0)
(16.68,0)
(16.69,0)
(16.7,0)
(16.71,0)
(16.72,0)
(16.73,0)
(16.74,0)
(16.75,0)
(16.76,1)
(16.77,1)
(16.78,1)
(16.79,1)
(16.8,1)
(16.81,1)
(16.82,1)
(16.83,1)
(16.84,1)
(16.85,1)
(16.86,1)
(16.87,1)
(16.88,1)
(16.89,1)
(16.9,1)
(16.91,1)
(16.92,1)
(16.93,1)
(16.94,1)
(16.95,1)
(16.96,1)
(16.97,1)
(16.98,1)
(16.99,1)
(17,1)
(17.01,1)
(17.02,1)
(17.03,1)
(17.04,1)
(17.05,1)
(17.06,1)
(17.07,1)
(17.08,1)
(17.09,1)
(17.1,1)
(17.11,1)
(17.12,1)
(17.13,1)
(17.14,1)
(17.15,1)
(17.16,1)
(17.17,1)
(17.18,1)
(17.19,1)
(17.2,1)
(17.21,1)
(17.22,1)
(17.23,1)
(17.24,1)
(17.25,1)
(17.26,1)
(17.27,1)
(17.28,1)
(17.29,1)
(17.3,1)
(17.31,1)
(17.32,1)
(17.33,1)
(17.34,1)
(17.35,1)
(17.36,1)
(17.37,1)
(17.38,1)
(17.39,1)
(17.4,1)
(17.41,1)
(17.42,1)
(17.43,1)
(17.44,1)
(17.45,1)
(17.46,1)
(17.47,1)
(17.48,1)
(17.49,1)
(17.5,1)
(17.51,1)
(17.52,1)
(17.53,1)
(17.54,0)
(17.55,0)
(17.56,0)
(17.57,0)
(17.58,0)
(17.59,0)
(17.6,0)
(17.61,0)
(17.62,0)
(17.63,0)
(17.64,0)
(17.65,0)
(17.66,0)
(17.67,0)
(17.68,0)
(17.69,0)
(17.7,0)
(17.71,0)
(17.72,0)
(17.73,0)
(17.74,0)
(17.75,0)
(17.76,0)
(17.77,0)
(17.78,0)
(17.79,0)
(17.8,0)
(17.81,0)
(17.82,0)
(17.83,0)
(17.84,0)
(17.85,0)
(17.86,0)
(17.87,0)
(17.88,0)
(17.89,0)
(17.9,0)
(17.91,0)
(17.92,0)
(17.93,0)
(17.94,0)
(17.95,0)
(17.96,0)
(17.97,0)
(17.98,0)
(17.99,0)
(18,0)
(18.01,0)
(18.02,0)
(18.03,0)
(18.04,0)
(18.05,0)
(18.06,0)
(18.07,0)
(18.08,0)
(18.09,0)
(18.1,0)
(18.11,0)
(18.12,0)
(18.13,0)
(18.14,0)
(18.15,0)
(18.16,0)
(18.17,0)
(18.18,0)
(18.19,0)
(18.2,0)
(18.21,0)
(18.22,0)
(18.23,0)
(18.24,0)
(18.25,0)
(18.26,0)
(18.27,0)
(18.28,0)
(18.29,0)
(18.3,0)
(18.31,0)
(18.32,0)
(18.33,0)
(18.34,0)
(18.35,0)
(18.36,0)
(18.37,0)
(18.38,0)
(18.39,0)
(18.4,0)
(18.41,0)
(18.42,0)
(18.43,0)
(18.44,0)
(18.45,0)
(18.46,0)
(18.47,0)
(18.48,0)
(18.49,0)
(18.5,0)
(18.51,0)
(18.52,0)
(18.53,0)
(18.54,0)
(18.55,0)
(18.56,0)
(18.57,0)
(18.58,0)
(18.59,0)
(18.6,0)
(18.61,0)
(18.62,0)
(18.63,0)
(18.64,0)
(18.65,0)
(18.66,0)
(18.67,0)
(18.68,0)
(18.69,0)
(18.7,0)
(18.71,0)
(18.72,0)
(18.73,0)
(18.74,0)
(18.75,0)
(18.76,0)
(18.77,0)
(18.78,0)
(18.79,0)
(18.8,0)
(18.81,0)
(18.82,0)
(18.83,0)
(18.84,0)
(18.85,0)
(18.86,0)
(18.87,0)
(18.88,0)
(18.89,0)
(18.9,0)
(18.91,0)
(18.92,0)
(18.93,0)
(18.94,0)
(18.95,0)
(18.96,0)
(18.97,0)
(18.98,0)
(18.99,0)
(19,0)
(19.01,0)
(19.02,0)
(19.03,0)
(19.04,0)
(19.05,0)
(19.06,0)
(19.07,0)
(19.08,0)
(19.09,0)
(19.1,0)
(19.11,0)
(19.12,0)
(19.13,0)
(19.14,0)
(19.15,0)
(19.16,0)
(19.17,0)
(19.18,0)
(19.19,0)
(19.2,0)
(19.21,0)
(19.22,0)
(19.23,0)
(19.24,0)
(19.25,0)
(19.26,0)
(19.27,0)
(19.28,0)
(19.29,0)
(19.3,0)
(19.31,0)
(19.32,0)
(19.33,0)
(19.34,0)
(19.35,0)
(19.36,0)
(19.37,0)
(19.38,0)
(19.39,0)
(19.4,0)
(19.41,0)
(19.42,0)
(19.43,0)
(19.44,0)
(19.45,0)
(19.46,0)
(19.47,0)
(19.48,0)
(19.49,0)
(19.5,0)
(19.51,0)
(19.52,0)
(19.53,0)
(19.54,0)
(19.55,0)
(19.56,0)
(19.57,0)
(19.58,0)
(19.59,0)
(19.6,0)
(19.61,0)
(19.62,0)
(19.63,0)
(19.64,0)
(19.65,0)
(19.66,0)
(19.67,0)
(19.68,0)
(19.69,0)
(19.7,0)
(19.71,0)
(19.72,0)
(19.73,0)
(19.74,0)
(19.75,0)
(19.76,0)
(19.77,0)
(19.78,0)
(19.79,0)
(19.8,0)
(19.81,0)
(19.82,0)
(19.83,0)
(19.84,0)
(19.85,0)
(19.86,0)
(19.87,0)
(19.88,0)
(19.89,0)
(19.9,0)
(19.91,0)
(19.92,0)
(19.93,0)
(19.94,0)
(19.95,0)
(19.96,0)
(19.97,0)
(19.98,0)
(19.99,0)
(20,0)
(20.01,0)
(20.02,0)
(20.03,0)
(20.04,0)
(20.05,0)
(20.06,0)
(20.07,0)
(20.08,0)
(20.09,0)
(20.1,0)
(20.11,0)
(20.12,0)
(20.13,0)
(20.14,0)
(20.15,0)
(20.16,0)
(20.17,0)
(20.18,0)
(20.19,0)
(20.2,0)
(20.21,0)
(20.22,0)
(20.23,0)
(20.24,0)
(20.25,0)
(20.26,0)
(20.27,0)
(20.28,0)
(20.29,0)
(20.3,0)
(20.31,0)
(20.32,0)
(20.33,0)
(20.34,0)
(20.35,0)
(20.36,0)
(20.37,0)
(20.38,0)
(20.39,0)
(20.4,0)
(20.41,0)
(20.42,0)
(20.43,0)
(20.44,0)
(20.45,0)
(20.46,0)
(20.47,0)
(20.48,0)
(20.49,0)
(20.5,0)
(20.51,0)
(20.52,0)
(20.53,0)
(20.54,0)
(20.55,0)
(20.56,0)
(20.57,0)
(20.58,0)
(20.59,0)
(20.6,0)
(20.61,0)
(20.62,0)
(20.63,0)
(20.64,0)
(20.65,0)
(20.66,0)
(20.67,0)
(20.68,0)
(20.69,0)
(20.7,0)
(20.71,0)
(20.72,0)
(20.73,0)
(20.74,0)
(20.75,0)
(20.76,0)
(20.77,0)
(20.78,0)
(20.79,0)
(20.8,0)
(20.81,0)
(20.82,0)
(20.83,0)
(20.84,0)
(20.85,0)
(20.86,0)
(20.87,0)
(20.88,0)
(20.89,0)
(20.9,0)
(20.91,0)
(20.92,0)
(20.93,0)
(20.94,0)
(20.95,0)
(20.96,0)
(20.97,0)
(20.98,0)
(20.99,0)
(21,0)
(21.01,0)
(21.02,0)
(21.03,0)
(21.04,0)
(21.05,0)
(21.06,0)
(21.07,0)
(21.08,0)
(21.09,0)
(21.1,0)
(21.11,0)
(21.12,0)
(21.13,0)
(21.14,0)
(21.15,0)
(21.16,0)
(21.17,0)
(21.18,0)
(21.19,0)
(21.2,0)
(21.21,0)
(21.22,0)
(21.23,0)
(21.24,0)
(21.25,0)
(21.26,0)
(21.27,0)
(21.28,0)
(21.29,0)
(21.3,0)
(21.31,0)
(21.32,0)
(21.33,0)
(21.34,0)
(21.35,0)
(21.36,0)
(21.37,0)
(21.38,0)
(21.39,0)
(21.4,0)
(21.41,0)
(21.42,0)
(21.43,0)
(21.44,0)
(21.45,0)
(21.46,0)
(21.47,0)
(21.48,0)
(21.49,0)
(21.5,0)
(21.51,0)
(21.52,0)
(21.53,0)
(21.54,0)
(21.55,0)
(21.56,0)
(21.57,0)
(21.58,0)
(21.59,0)
(21.6,0)
(21.61,0)
(21.62,0)
(21.63,0)
(21.64,0)
(21.65,0)
(21.66,0)
(21.67,0)
(21.68,0)
(21.69,0)
(21.7,0)
(21.71,0)
(21.72,0)
(21.73,0)
(21.74,0)
(21.75,0)
(21.76,0)
(21.77,0)
(21.78,0)
(21.79,0)
(21.8,0)
(21.81,0)
(21.82,0)
(21.83,0)
(21.84,0)
(21.85,0)
(21.86,0)
(21.87,0)
(21.88,0)
(21.89,0)
(21.9,0)
(21.91,0)
(21.92,0)
(21.93,0)
(21.94,0)
(21.95,0)
(21.96,0)
(21.97,0)
(21.98,0)
(21.99,0)
(22,0)
(22.01,0)
(22.02,0)
(22.03,0)
(22.04,0)
(22.05,0)
(22.06,0)
(22.07,0)
(22.08,0)
(22.09,0)
(22.1,0)
(22.11,0)
(22.12,0)
(22.13,0)
(22.14,0)
(22.15,0)
(22.16,0)
(22.17,0)
(22.18,0)
(22.19,0)
(22.2,0)
(22.21,0)
(22.22,0)
(22.23,0)
(22.24,0)
(22.25,0)
(22.26,0)
(22.27,0)
(22.28,0)
(22.29,0)
(22.3,0)
(22.31,0)
(22.32,0)
(22.33,0)
(22.34,0)
(22.35,0)
(22.36,0)
(22.37,0)
(22.38,0)
(22.39,0)
(22.4,0)
(22.41,0)
(22.42,0)
(22.43,0)
(22.44,0)
(22.45,0)
(22.46,0)
(22.47,0)
(22.48,0)
(22.49,0)
(22.5,0)
(22.51,0)
(22.52,0)
(22.53,0)
(22.54,0)
(22.55,0)
(22.56,0)
(22.57,0)
(22.58,0)
(22.59,0)
(22.6,0)
(22.61,0)
(22.62,0)
(22.63,0)
(22.64,0)
(22.65,0)
(22.66,0)
(22.67,0)
(22.68,0)
(22.69,0)
(22.7,0)
(22.71,0)
(22.72,0)
(22.73,0)
(22.74,0)
(22.75,0)
(22.76,0)
(22.77,0)
(22.78,0)
(22.79,0)
(22.8,0)
(22.81,0)
(22.82,0)
(22.83,0)
(22.84,0)
(22.85,0)
(22.86,0)
(22.87,0)
(22.88,0)
(22.89,0)
(22.9,0)
(22.91,0)
(22.92,0)
(22.93,0)
(22.94,0)
(22.95,0)
(22.96,0)
(22.97,0)
(22.98,0)
(22.99,0)
(23,0)
(23.01,0)
(23.02,0)
(23.03,0)
(23.04,0)
(23.05,0)
(23.06,0)
(23.07,0)
(23.08,0)
(23.09,0)
(23.1,0)
(23.11,0)
(23.12,0)
(23.13,0)
(23.14,0)
(23.15,0)
(23.16,0)
(23.17,0)
(23.18,0)
(23.19,0)
(23.2,0)
(23.21,0)
(23.22,0)
(23.23,0)
(23.24,0)
(23.25,0)
(23.26,0)
(23.27,0)
(23.28,0)
(23.29,0)
(23.3,0)
(23.31,0)
(23.32,0)
(23.33,0)
(23.34,0)
(23.35,0)
(23.36,0)
(23.37,0)
(23.38,0)
(23.39,0)
(23.4,0)
(23.41,0)
(23.42,0)
(23.43,0)
(23.44,0)
(23.45,0)
(23.46,0)
(23.47,0)
(23.48,0)
(23.49,0)
(23.5,0)
(23.51,0)
(23.52,0)
(23.53,0)
(23.54,0)
(23.55,0)
(23.56,0)
(23.57,0)
(23.58,0)
(23.59,0)
(23.6,0)
(23.61,0)
(23.62,0)
(23.63,0)
(23.64,0)
(23.65,0)
(23.66,0)
(23.67,0)
(23.68,0)
(23.69,0)
(23.7,0)
(23.71,0)
(23.72,0)
(23.73,0)
(23.74,0)
(23.75,0)
(23.76,0)
(23.77,0)
(23.78,0)
(23.79,0)
(23.8,0)
(23.81,0)
(23.82,0)
(23.83,0)
(23.84,0)
(23.85,0)
(23.86,0)
(23.87,0)
(23.88,0)
(23.89,0)
(23.9,0)
(23.91,0)
(23.92,0)
(23.93,0)
(23.94,0)
(23.95,0)
(23.96,0)
(23.97,0)
(23.98,0)
(23.99,0)
(24,0)
(24.01,0)
(24.02,0)
(24.03,0)
(24.04,0)
(24.05,0)
(24.06,0)
(24.07,0)
(24.08,0)
(24.09,0)
(24.1,0)
(24.11,0)
(24.12,0)
(24.13,0)
(24.14,0)
(24.15,0)
(24.16,0)
(24.17,0)
(24.18,0)
(24.19,0)
(24.2,0)
(24.21,0)
(24.22,0)
(24.23,0)
(24.24,0)
(24.25,0)
(24.26,0)
(24.27,0)
(24.28,0)
(24.29,0)
(24.3,0)
(24.31,0)
(24.32,0)
(24.33,0)
(24.34,0)
(24.35,0)
(24.36,0)
(24.37,0)
(24.38,0)
(24.39,0)
(24.4,0)
(24.41,0)
(24.42,0)
(24.43,0)
(24.44,0)
(24.45,0)
(24.46,0)
(24.47,0)
(24.48,0)
(24.49,0)
(24.5,0)
(24.51,0)
(24.52,0)
(24.53,0)
(24.54,0)
(24.55,0)
(24.56,0)
(24.57,0)
(24.58,0)
(24.59,0)
(24.6,0)
(24.61,0)
(24.62,0)
(24.63,0)
(24.64,0)
(24.65,0)
(24.66,0)
(24.67,0)
(24.68,0)
(24.69,0)
(24.7,0)
(24.71,0)
(24.72,0)
(24.73,0)
(24.74,0)
(24.75,0)
(24.76,0)
(24.77,0)
(24.78,0)
(24.79,0)
(24.8,0)
(24.81,0)
(24.82,0)
(24.83,0)
(24.84,0)
(24.85,0)
(24.86,0)
(24.87,0)
(24.88,0)
(24.89,0)
(24.9,0)
(24.91,0)
(24.92,0)
(24.93,0)
(24.94,0)
(24.95,0)
(24.96,0)
(24.97,0)
(24.98,0)
(24.99,0)
	};
